Provably Efficient Sample Complexity for Robust CMDP

We study the problem of learning policies that maximize cumulative reward while satisfying safety constraints, even when the real environment differs from a simulator or nominal model. We focus on robust constrained Markov decision processes (RCMDPs), where the agent must maximize reward while ensuring cumulative utility exceeds a threshold under the worst-case dynamics within an uncertainty set. While recent works have established finite-time iteration complexity guarantees for RCMDPs using policy optimization, their sample complexity guarantees remain largely unexplored. In this paper, we first show that Markovian policies may fail to be optimal even under rectangular uncertainty sets unlike the {\em unconstrained} robust MDP. To address this, we introduce an augmented state space that incorporates the remaining utility budget into the state representation. Building on this formulation, we propose a novel Robust constrained Value iteration (RCVI) algorithm with a sample complexity of $\mathcal{\tilde{O}}(|S||A|H^5/\epsilon^2)$ achieving at most $\epsilon$ violation using a generative model where $|S|$ and $|A|$ denote the sizes of the state and action spaces, respectively, and $H$ is the episode length. To the best of our knowledge, this is the {\em first sample complexity guarantee} for RCMDP. Empirical results further validate the effectiveness of our approach.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction appropriately talk about our contribution.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}%{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our limitations are clearly stated in the main text
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the assumptions in the main text and the proofs of lemmas in the supplementary section
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The complete set of hyperparameters are given in the supplementary section also the environments are discussed in details under Implementation details in the appendix
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The complete set of hyperparameters are given in the supplementary section also the environments are discussed in details under Implementation details in the appendix
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It is an simulation, we do not need test-train splitting of data
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Such estimations were not required here
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It is mentioned in the appendix. Also, whether hardware accelerators were used or not is disclosed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It follows them.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This discussion is not applicable to our work
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The environments are simulated so no need for these description
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We comply with this.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper clearly states them.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Crowd sourcing was not required
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No participants were needed for our work
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work does not derive any help from LLMs apart from the spell-check and formatting.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> complete_experiment_details.tex <==
\subsection{Experiments}
\label{app:experiments}
The experiments were performed on two very popular benchmarks in RL\footnote{Lower threshold experiments ($b=4.5$ for RCVI in CRS) were done in colab without use of hardware accelerators such as GPU or TPU for higher threshold $b=30$ for CRS and for Garnet are done in a local machine, having 4GB RAM and 1 TB of hard disk, no GPU support is necessary.} (i) Constrained River-swim (CRS) and (ii) Cost-based Garnet environment. For both the experiments, the f-divergence metric is assumed to be KL-divergence. Although the algorithm is not limited to KL-divergence and can be extended to other f-divergence measures such as TV-distance, $\chi^{2}$-distribution etc.  There are two important reasons for choosing the KL-divergence over the other f-divergence metrics. First the existence of a closed form evaluation method that makes the robust policy evaluation having a known nominal model ($P_{0}$), simple (see Appendix \ref{kl_divergence}). Secondly, the KL-divergence is very stable with minimum influence of the changing hyperparameters. The uncertainty is introduced in both environments by adding noise to the nominal model transition probabilities and then normalizing them to make a probability distribution during training time and by reversing the probability distribution in the testing or inference time.

\subsection{Constrained River-swim}
The constrained River-swim (CRS) is an important benchmark environment studied in optimization theory and control. We briefly introduce the objective of the Constrained River-swim environment, followed by the results obtained upon training our algorithm (Algorithm \ref{algo:rs-cmdp}) on CRS.

\subsubsection{Environment Description}
The environment consists of $6$ states, each representing a landmass.  A swimmer starts in one of these states according to a random initial distribution.  At any state, the swimmer can choose between two actions: \emph{swim left} ($a_{0}$) or \emph{swim right} ($a_{1}$).  Each action leads to a probabilistic transition to the next state, governed by a transition distribution.  

The swimmer receives rewards only at the extreme states (in this case, $s_{0}$ and $s_{5}$).  However, the environment also introduces risks:  
\begin{itemize}
    \item A \textbf{river current} always pushes against the swimmer’s chosen direction, making movement more uncertain.  
    \item \textbf{Harmful creatures} inhabit the landmasses, causing injury to the swimmer. The number of these creatures increases as we move to higher-indexed states.  
\end{itemize}

Thus, $s_{0}$ is the safest state with minimal reward and minimal cost, while states with larger indices carry linearly increasing costs due to greater safety hazards.  The swimmer’s objective is to learn an optimal policy that balances reward and safety, despite uncertainties in the transition dynamics, given only a nominal transition probability distribution $P_{0}$.

\subsubsection{Implementation details}
Constrained River-swim environment consists of $6$ states so, let us denote the six states as $\mathcal{S} = \{s_{0},s_{1},s_{2},\ldots,s_{5}\}$ and $2$ actions denoted as $\mathcal{A} =\{a_{0},a_{1} \}$ where $\mathcal{S}$ and $\mathcal{A}$ denotes the state space and action space respectively. We consider a six-state RiverSwim environment with states $\mathcal{S}={s_0,\ldots,s_5}$ and actions $\mathcal{A}={a_0,a_1}$. For $s_i$, $i=1,\ldots,5$, action $a_0$ transitions to $(s_i,s_{i-1},s_{i+1})$ with probabilities $(0.6,0.3,0.1)$, while for $i=0,\ldots,4$, action $a_1$ transitions to $(s_i,s_{i-1},s_{i+1})$ with probabilities $(0.6,0.1,0.3)$, with the boundary transitions $P(s_0|s_0,a_0)=P(s_5|s_5,a_1)=0.9$. The state-wise reward and constraint cost are $(r,c)={(0.001,0.02),(0,0.035),(0,0),(0,0.01),(0.1,0.08),(1,0.9)}$ for $s_0,\ldots,s_5$, respectively. 

For the CRS experiments, we set the budget to $B=4.5$, with $|\mathcal{S}|=6$ states and $|\mathcal{A}|=2$ actions. The algorithm is configured with $10$ bins, an $f$-divergence tolerance of $\rho=0.05$, a horizon length of $H=1000$, and a sample size of $N=1000$.


\subsubsection{Additional Results and discussion}
% The results obtained upon training Algorithm \ref{algo:rs-cmdp} on CRS is as shown in figures \ref{fig:CRS_vf_app} and \ref{fig:CRS_cf_app}
In addition to the experiments reported in Figure~\ref{fig:crs_ib_cf_vf_main}, we conduct several supplementary experiments to further illustrate the limitations of the Markovian policy setup and the advantages of the augmented formulation.

The choice of budget threshold $b=4.5$ may appear unconventional and could raise questions regarding its selection. Our motivation, however, is deliberate: we choose $b$ so that none of the competing algorithms can identify a feasible policy under this budget. This helps expose a fundamental limitation of the Markovian setup, namely its inability to recover feasible policies when all candidate policies lie in the unsafe region, a limitation that does not arise in the augmented setting.

%As an alternative way to demonstrate this phenomenon, we also increase the cost at every state by $0.5$. Figures~\ref{fig:CRS_vf_app}, \ref{fig:CRS_cf_app}, \ref{fig:CRS_app_inc_cost_vf}, and \ref{fig:CRS_app_inc_cost_cf} show the results for this modified cost function relative to the costs reported in Table~\ref{tab:rs_r_c}. \textcolor{red}{Note that we omit RRPO and EPIRC-PGS from these plots because their values were too close to distinguish clearly.}

%The reason RCVI does not violate the threshold in either setup stems from its discretization of cost budget over the range $[0,b]$. Since RCVI only permits decisions within this discretized budget space, the agent cannot select actions that lead beyond the prescribed cost bound. In contrast, the other algorithms do not impose any analogous budget discretization or bucket structure and instead update parameters iteratively without an explicit mechanism guaranteeing feasibility. Consequently, when all candidate policies lie in the unsafe region, these methods have no way to recover a feasible policy. %To explicitly demonstrate this limitation, we choose the challenging threshold $b=4.5$ in Figures~\ref{fig:crs_ib_cf_vf_main} and \ref{fig:CRS_app_list}.

% \begin{figure}
%     \centering
%     \begin{subfigure}
%         \includegraphics[]{images/Aistats_VI_vf.pdf}
%         \caption{The value function at each iteration step}
%         \label{fig:CRS_vf}
%     \end{subfigure}

%     \begin{subfigure}
%         \includegraphics[]{images/Aistats_VI_cf.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:CRS_cf}
%     \end{subfigure}
%     \caption{The worst case value function and cost function update at each iteration step where the x-axis denotes the Iteration number and the y-axis denots the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) denoted as Robust value function and Robust cost function respectively.}
%     \label{fig:CRS}
% \end{figure}

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[clip=2in 2in 2in 2in,height=2.3in]{images/Comparison_plots_rho_1e-1_baseline_reducedCRSvf.pdf}
%          \caption{The value function at each iteration step}
%         \label{fig:CRS_vf_app}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[clip=2in 2in 2in 2in,height=2.3in]{images/Comparison_plots_rho_1e-1_baseline_reducedCRSCF.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:CRS_cf_app}
%     \end{subfigure}
%     \caption{The Robust value function and Robust cost function update (CRS environment) at each iteration step , the baseline kept as 5 and cost at each step is increased by $0.5$ with respect to table \ref{tab:rs_r_c} ($\rho=0.01$)}
%     \label{fig:CRS_app_1}
% \end{figure*}

% The baseline for the cost function ($b$) or the budget was fixed at $4.5$.  As seen in figure \ref{fig:CRS_vf_app}, the value function steadily increases to the maximum possible in the given budget range. Starting from $0.24$ approximately which denotes the robust value function for the policy of equiprobable actions in each states (i.e $\pi(a|s) = \frac{1}{|\mathcal{A}|}~\forall s\in \mathcal{S}$), it slowly increases and after 50 iterations it converges to the policy where the robust value function is maximum. As it is evident that the convergence is faster compared to other state-of-the approaches. Further, the RCVI (Algorithm~\ref{algo:rs-cmdp}) is always feasible.   The implementation details along with the hyperparameters are listed in the following subsection. %(Since, the baseline staright line and the RCVI cost function plot is nearly coinciding refer to figure \ref{zoom_in_CRS_cf} for better demonstration).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{images/Comparison_plots_rho_1e-1_inc_cost_zoom_CRSCF.pdf}
%     \caption{Robust cost function update at each iteration on CRS environment (baseline =4.5 and zoomed in to show how many times RCVI cost function goes past the baseline)}
%     \label{zoom_in_CRS_cf}
% \end{figure}

%In another set of experiments on CRS environment, we increased the baseline by $0.5$, that is the new baseline was set at $5$ (we also ran one set of experiment by fixing the baseline at 7 and keeping all other hyper-parameters, rewards and cost intact as this experiment and results were almost similar). However, we increased the cost at each state denoted by Table \ref{tab:rs_r_c} by $0.5$. This experiment was performed as a control experiment to verify if RNPG or RCRPO perform in par with RCVI. The results of which are depicted in figures \ref{fig:CRS_app_inc_cost_vf} and \ref{fig:CRS_app_inc_cost_cf}.

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[clip=2in 2in 2in 2in,height=2.3in]{images/Comparison_plots_rho_1e-2_increased_costCRSvf.pdf}
%          \caption{The value function at each iteration step}
%         \label{fig:CRS_app_inc_cost_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[clip=2in 2in 2in 2in,height=2.3in]{images/Comparison_plots_rho_1e-2_increased_costCRSCF.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:CRS_app_inc_cost_cf}
%     \end{subfigure}
%     \caption{\small The Robust value function and Robust cost function update (CRS environment) at each iteration step , the baseline kept as 5 and cost at each step is increased by $0.5$ with respect to table \ref{tab:rs_r_c} ($\rho=0.1$)}
%     \label{fig:CRS_app_2}
% \end{figure*}

\paragraph{Test Time  results} 
\label{testing_CRS}
Since our training procedure incorporates robustness, it is important to verify whether these benefits persist at inference (test) time under perturbed dynamics. To evaluate this, we deliberately perturb the transition probabilities during testing. Specifically, if the agent is at state $s_t=x$, it can transition to one of $s_{t+1}=\{x-1,x,x+1\}$ with probabilities $p_1,p_2,p_3$, respectively. During testing, with probability $\epsilon$, we randomly alter the transition ordering; for example, the transition probabilities may change from $(p_1,p_2,p_3)$ to $(p_3,p_2,p_1)$. For our test-time, we set $\epsilon=0.05$.

 We initialize from random states, sample actions from the learned Q-table using the same cost discretization, and run a reduced evaluation over $100$ independent episodes. We then report the average robust value function and robust cost function, summarized in Table~\ref{tab:robust_results}.
% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|}
%     \hline
%         \textbf{Environment name}&\textbf{RCVI} &RNPG&RRPO&EPIRC-PGS&RCRPO  \\
%         \hline
%         \textit{CRS}&\textbf{5.5044} &6.0456&5.00031& 14.113&12.7812\\
%         \hline
%          \textit{Garnet}&\textbf{4.4081}&8.2304&6.00214&9.211&11.5488 \\
%          \hline
%     \end{tabular}
%     \caption{Average robust value functions of 100 steps for all the algorithms on the two environments}
%     \label{tab:testing_vf}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%         \textbf{RCVI} &RNPG&RRPO&EPIRC-PGS&RCRPO   \\
%         \hline
%          \textit{CRS}&\textbf{4.4081}&8.2304&6.00214&9.211&11.5488 \\
%          \hline
         
%     \end{tabular}
%     \caption{Average robust cost functions of 100 steps for all the algorithms,  $b=4.5$.}
%     \label{tab:testing_cf_CRS}
% \end{table}
\subsubsection{Training with an increased safety threshold value}
% \paragraph{Training with a safety threshold $b=7$} In addition to the above setup, we run our algorithm with a higher safety threshold value to underscore the performance of RCVI. We first consider $b=7$ and $\rho=0.1$.  Since $b$ is high, now the Markovian policies in the original state-space is feasible, yet we observe that our proposed approach (RCVI) converges faster compared to the other baselines (Figure~\ref{fig:one_safe_pol_crs}).   From Figure \ref{one_safe_pol_crs_vf}, we note that all the algorithms have comparable value functions, and Figure \ref{one_safe_pol_crs_cf} tells us that all the algorithms are in the safe zone. %Hence, we can conclude that RCVI  returns a high-returning (comparable to other baselines) feasible policy.

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.2in]{images/Baseline_where_one_policy_in_safe_zone_vf_CRS.pdf}
%          \caption{The value function at each iteration step}
%         \label{one_safe_pol_crs_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.2in]{Baseline_where_one_policy_in_safe_zone_cf_CRS.pdf}
%         \caption{The cost function at each iteration step}
%         \label{one_safe_pol_crs_cf}
%     \end{subfigure}
%     \caption{\small Robust value function and cost function update at each iteration on Constrained River-swim(CRS environment) $b=7$.}
%     %\vspace-0.2in}
%     \label{fig:one_safe_pol_crs}
% \end{figure*}

% \paragraph{Training with a safety threshold $b=30$}
In addition to the above setup, we run our algorithm with a higher safety threshold value to underscore the performance of RCVI. We consider threshold $b=30$ and $\rho=0.1$. Here, the Markovian policy in the original state-space is feasible, and all the other baselines converge to the optimal policy as well. In this setup too, we find that the convergence of RCVI is faster compared to other state-of-the-art approaches (Figure~\ref{fig:crs_ib_cf_vf}. RCVI also achieves a similar reward while maintaining feasibility throughout the training. {\em This set of studies  tell us that RCVI can  not only find a feasible policy but also the highest-returning feasible policy across different values of $b$}. Further, RCVI converges  faster compared to  all the state-of-the-art approaches.  
\begin{figure*}[h!]
    \centering
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Value_function_plot_for_safe_initial_policy_CRS_b=30.pdf}
         \caption{The value function at each iteration step}
        \label{fig:crs_ib_vf}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Cost_function_plot_for_safe_initial_policy_CRS_b=30.pdf}
        \caption{The cost function at each iteration step}
        \label{fig:crs_ib_cf}
    \end{subfigure}
    \caption{\small Robust value function and cost function update at each iteration on Constrained River-swim (CRS) environment for $b=30$.}
    \label{fig:crs_ib_cf_vf}
\end{figure*}
%\vspace-0.1in}
\subsubsection{Ablation study on uncertainty measure $\rho$}
In this section, we perform an ablation study on different values of $\rho$ for the CRS environment (original setting). The results of which can be found in Figure \ref{fig:CRS_app_list} where we compare with the baselines.

\begin{figure*}[]
    \centering
    \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.01_vf.pdf}
         \caption{The value function at each iteration step ($\rho=0.01$)}
        \label{fig:CRS_vf_app_0.01}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.01_cf.pdf}
        \caption{The cost function at each iteration step ($\rho=0.01$)}
        \label{fig:CRS_cf_app_0.01}
    \end{subfigure}%
    \\
    \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.05_vf.pdf}
        \caption{The value function at each iteration step($\rho=0.05$)}
        \label{fig:CRS_vf_app_0.05}
    \end{subfigure}%
    ~
    \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.05_cf.pdf}
        \caption{The cost function at each iteration step($\rho=0.05$)}
        \label{fig:CRS_cf_app_0.05}
    \end{subfigure}%
    \\
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.1_vf.pdf}
         \caption{The value function at each iteration step($\rho=0.1$)}
        \label{fig:CRS_vf_app_0.1}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.1_cf.pdf}
        \caption{The cost function at each iteration step($\rho=0.1$)}
        \label{fig:CRS_cf_app_0.1}
    \end{subfigure}
    %  \begin{subfigure}[]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=2.3in]{images/Abalation_CRS_rho_0.05_vf.pdf}
    %      \caption{The value function at each iteration step ($\rho=0.05$)}
    %     \label{fig:CRS_vf_app_0.1}
    % \end{subfigure}%
    % ~ 
    % \begin{subfigure}[]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=2.3in]{images/Ablataion_CRS_rho_0.05_cf.pdf}
    %     \caption{The cost function at each iteration step ($\rho=0.05$)}
    %     \label{fig:CRS_cf_app_0.1}
    % \end{subfigure}%
   % \begin{subfigure}[h]{0.5\textwidth}
   %      \centering
   %      \includegraphics[height=2.8in]{images/Aistats_VI_vf_Garnet.pdf}
   %       \caption{The value function at each iteration step }
   %      \label{app:fig_gar_vf}
   %  \end{subfigure}%
   %  ~ 
   %  \begin{subfigure}[h]{0.5\textwidth}
   %      \centering
   %      \includegraphics[height=2.8in]{images/Aistats_VI_cf_Garnet.pdf}
   %      \caption{The cost function at each iteration step($\rho=0.5$)}
   %      \label{app:fig_gar_cf}
   %  \end{subfigure}
    \caption{\small The x-axis denotes the Iteration number and the y-axis denotes the worst case reward value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) for various algorithms on the CRS environment for different values of $\rho$.}
    \label{fig:CRS_app_list}
\end{figure*}

The first row of plots (Figures~\ref{fig:CRS_vf_app_0.01} and~\ref{fig:CRS_cf_app_0.01}) corresponds to $\rho = 0.01$, the following row of plots correspond to $\rho = 0.05$ (Figures~\ref{fig:CRS_vf_app_0.05} and~\ref{fig:CRS_cf_app_0.05}) and the final row (Figures~\ref{fig:CRS_vf_app_0.1} and~\ref{fig:CRS_cf_app_0.1}) of plots correspond to $\rho=0.1$. The baseline was kept at $4.5$ for all the experiments. In all cases, baseline algorithms such as RNPG, RRPO, RCRPO, and EPIRC-PGS operate in the unsafe region, requiring large iterations to converge. In contrast, our RCVI algorithm consistently remains within the safe boundary,  and converges to the optimal policy quickly.% Moreover, for $\rho=0.1$ (Figure~\ref{fig:CRS_vf_app_0.1}) the achieved value function is slightly higher compared to RNPG.

\subsection{Cost-based Garnet problem}
The Garnet problem is another fundamental benchmark problem used in Control theory and Reinforcement Learning to test the effectiveness of an algorithm. In the next subsection we briefly discuss about the environment with the results in the following subsection
\subsubsection{Environment Description}
The \emph{Garnet environment} is a widely used MDP benchmark designed for evaluating RL algorithms under controlled conditions. 
It is defined by a fixed number of states \(nS\) and actions \(nA\), with transition probabilities, rewards, and (in constrained RL) utility functions sampled from prescribed distributions. 
A key feature of the Garnet setup is that the transition dynamics are typically \emph{sparse}, meaning that each state--action pair leads only to a limited subset of possible successor states rather than all states.  

Formally, the environment is specified by a transition probability kernel \(P(s' \mid s, a)\), a reward function \(R(s, a)\), and, when applicable, a utility function \(U(s, a)\). 
These quantities are often sampled from normal distributions:
\begin{align*}
P(s' \mid s, a) \sim \mathcal{N}(\mu_a, \sigma_a),\\ 
R(s, a) \sim \mathcal{N}(\mu_b, \sigma_b),\\ 
 U(s, a) \sim \mathcal{N}(\mu_c, \sigma_c),
\end{align*}
where the means \(\mu_a, \mu_b, \mu_c\) are themselves drawn from a uniform distribution, i.e., 
\(\text{Unif}(0,10)\).  

Since \(P(s' \mid s, a)\) must define a valid probability distribution (each row summing to one), 
The sampled values are exponentiated and normalized via a softmax transformation:
\[
p^{0}(s' \mid s, a) 
= \frac{\exp(P(s' \mid s, a))}{\sum_{s''} \exp(P(s'' \mid s, a))}.
\]

However, our cost-based Garnet environment is a slightly changed version of the aforementioned environment. In this cost based setting, we assumed a cost function $C(s, a) \sim \mathcal{N}(\mu_{c},\sigma_{c})$ instead of the utility function $U(s, a)$ and the new objective of the cost based Garnet environment is to maximize the long term objective function while keeping the long term cost function denoted as $V_{P,c}^{\pi}=\sum_{t=1}^{T}\mathbb{E}_{P}\left[ C(s_{t},\pi_{t}(s_{t}))\right] \leq b$ below a certain threshold value $b$.

\subsubsection{Implementation details}
The Garnet environment had $10$ states denoted as $s_{0} \ldots s_{9}$ and $5$ distinct actions denoted as $a_{0} \ldots a_{4}$. For the Garnet experiments, we set the budget to $B=15$, with $|\mathcal{S}|=10$ states and $|\mathcal{A}|=5$ actions. The environment parameters $\mu_a,\mu_b,\mu_c$ and $\sigma_a,\sigma_b,\sigma_c$ are independently sampled from $\operatorname{Unif}(0,10)$. The algorithm is configured with $20$ bins, an $f$-divergence tolerance $\rho\in{0.05,0.01,0.1}$, a horizon length of $H=1000$, and a sample size of $N=1000$.
% \section{Additional experiments}
% \label{app:add_expt}

\subsubsection{Additional Results and discussion}
Similar to the CRS environment, we conduct additional experiments to support the advantages of our approach. The choice of budget for most of the pilot studies, the testing time study, and the ablation study was 15.
% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.2in]{Comparison_plots_rho_1e-1_icmlGarnetvf.pdf}
%          \caption{The value function at each iteration step}
%         \label{app:fig_gar_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.2in]{Comparison_plots_rho_1e-1_icmlGarnetCF.pdf}
%         \caption{The cost function at each iteration step}
%         \label{app:fig_gar_cf}
%     \end{subfigure}
%     \caption{The worst case value function and cost function (garnet environment) update at each iteration step where the x-axis denotes the Iteration number and the y-axis denotes the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) with the cost at each state randomly increased by $Unif(0,0.5)$.}
%     \label{fig:garnet_app}
% \end{figure*}

\paragraph{Testing Time (Inference time) results}
\label{testing_garnet}
During test time, we run $100$ independent episodes where the initial state is chosen randomly. The average robust value function and average robust cost function are listed in tables \ref{tab:robust_results}. Only the RCVI achieves a feasible policy while also achieving a good reward. 



% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%         \textbf{RCVI} &RNPG&RRPO&EPIRC-PGS&RCRPO  \\
%         \hline
%         \textbf{21.0125} &22.9541&20.1546& 20.5441&31.1546\\
%         \hline
%     \end{tabular}
%     \caption{\small Average robust value functions of 100 steps for all the algorithms (Garnet environment)}
%     \label{tab:rvf_garnet}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%         \textbf{RCVI} &RNPG&RRPO&EPIRC-PGS&RCRPO   \\
%         \hline
%          \textbf{14.9562}&23.5541&19.8456&22.7741&24.1179 \\
%          \hline
         
%     \end{tabular}
%     \caption{\small Average robust cost functions of 100 steps for all the algorithms (Garnet environment), $b=15$.}
%     \label{tab:rcf_garnet}
% \end{table}
\subsubsection{Training with an increased safety threshold value}
% \paragraph{Training with a safety threshold $b=25$}  We begin by studying a slightly higher baseline $b=25$. The findings from this study are compiled in Figures \ref{one_safe_pol_garnet_vf} and \ref{one_safe_pol_garnet_cf}. 
% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.2in]{images/Baseline_where_one_policy_in_safe_zone_vf_garnet.pdf}
%          \caption{The value function at each iteration step}
%         \label{one_safe_pol_garnet_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.2in]{images/Baseline_where_one_policy_in_safe_zone_cf_garnet.pdf}
%         \caption{The cost function at each iteration step}
%         \label{one_safe_pol_garnet_cf}
%     \end{subfigure}
%     \caption{The above plot shows when only 1 policy exists in the feasible zone then all other algorithms finds that policy however, our RCVI algorithm is still effective in such situations (Garnet environment) $b=25$.}
%     \label{fig:one_safe_pol_garnet}
% \end{figure*}
% Since $b$ is high, the Markovian policies are also feasible. As observed from Figure \ref{fig:one_safe_pol_garnet}, all the algorithms converge to a close enough policy with  comparable value function and cost functions. However, our proposed approach RCVI coverges the fastest among all the other approaches. 

Similar to CRS, for this envionment too, we try with an elevated baseline value $b=50$. From Figure~\ref{fig:gar_ib_cf_vf} note that our proposed approach is the fastest among all the other approaches. The achieved reward is almost similar with the baselines while maintaining feasibility throughout the training. %The plots for this study is shown in figure \ref{fig:gar_ib_cf_vf}.

\begin{figure*}[h!]
    \centering
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[clip=2in 2in 2in 2in,height=2.3in]{images/Value_function_plot_for_safe_initial_policy_Garnet_b=50.pdf}
         \caption{The value function at each iteration step}
        \label{fig:gar_ib_vf}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[h]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Cost_function_plot_for_safe_initial_policy_Garnet_b=50.pdf}
        \caption{The cost function at each iteration step}
        \label{fig:gar_ib_cf}
    \end{subfigure}
    \caption{\small Robust value function and cost function update at each iteration on Garnet environment (b=50).}
    \label{fig:gar_ib_cf_vf}
\end{figure*}

%As seen from figure \ref{fig:gar_ib_cf_vf}, RCVI performs in par with other algorithms. Thus, we can draw the inference from this experiment that RCVI performs efficiently in large baseline conditions as well.

Evaluating both environments, despite their similar uncertainty estimators and indices, strengthens the robustness and generalizability of the results across different settings.

\subsubsection{Ablation study on uncertainty measure $\rho$}
%\vspace-0.1in}
Similar to the CRS setting, we conduct an ablation study on different values of $\rho$ for the Garnet environment. 
%The uncertainty parameter $\rho$ plays a crucial role in shaping the policy search space, as varying $\rho$ alters the set of admissible policies. To understand the impact of this hyperparameter, we systematically evaluate performance across different values of $\rho$. 
The corresponding results are presented in Figure \ref{fig:Garnet_app_list}.
%The cost budget was kept at 5, since higher values might require higher discretizations to perform best.  


\begin{figure*}[]
    \centering
    \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.01_vf.pdf}
         \caption{The value function at each iteration step ($\rho=0.01$)}
        \label{app:fig_gar_vf_0.01}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.01_cf.pdf}
        \caption{The cost function at each iteration step ($\rho=0.01$)}
        \label{app:fig_gar_cf_0.01}
    \end{subfigure}
    \\
    \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.05_vf.pdf}
         \caption{The value function at each iteration step ($\rho=0.05$)}
        \label{app:fig_gar_vf_0.05}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.05_cf.pdf}
        \caption{The cost function at each iteration step ($\rho=0.05$)}
        \label{app:fig_gar_cf_0.05}
    \end{subfigure}
    \\
     \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.1_vf.pdf}
         \caption{The value function at each iteration step ($\rho=0.1$)}
        \label{app:fig_gar_vf_0.1}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[]{0.5\textwidth}
        \centering
        \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.1_cf.pdf}
        \caption{The cost function at each iteration step ($\rho=0.1$)}
        \label{app:fig_gar_cf_0.1}
    \end{subfigure}
    % \begin{subfigure}[]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=2.3in]{images/Comparison_plots_rho_1e-1_Garnetvf.pdf}
    %      \caption{The value function at each iteration step ($\rho=0.1$)}
    %     \label{app:fig_gar_vf_0.1}
    % \end{subfigure}%
    % ~ 
    % \begin{subfigure}[]{0.5\textwidth}
    %     \centering
    %     \includegraphics[height=2.3in]{images/Comparison_plots_rho_1e-1_GarnetCF.pdf}
    %     \caption{The cost function at each iteration step ($\rho=0.1$)}
    %     \label{app:fig_gar_cf_0.1}
    % \end{subfigure}
    \caption{\small The worst case reward value function and cost function update at each iteration step where the x-axis denotes the Iteration number and the y-axis denotes the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure)  on the cost based Garnet environment.}
    \label{fig:Garnet_app_list}
\end{figure*}
% \subsection{More Experimental results}
%We further understand the working of our algorithm and here are the results obtained below
% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Value_function_plot_for_safe_initial_policy_CRS.pdf}
%          \caption{The value function at each iteration step}
%         \label{fig:crs_sp_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Cost_function_plot_for_safe_initial_policy_CRS.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:crs_sp_cf}
%     \end{subfigure}
%     \caption{The worst case value function and cost function update upon running our algorithm and other baselines on the CRS environment.}
%     \label{fig:crs_sp_cf_vf}
% \end{figure*}

Figures \ref{fig:Garnet_app_list} shows a detailed comparison when all the algorithms start from the safe zone, we see only RCVI converges to a safe feasible high returning policy due to its structure while others although start safe, after the parameters gets fixed, they converge to a non-feasible policy. This is because, the baseline was deliberately kept such that none of the policies could satisfy. Even for a higher value of $\rho$, RCVI can achieve a feasible policy while the other algorithms cannot.  %With very small learning rate too the agents quickly move out of safe zone. % A similar pattern is observed in the Garnet environment which is evident from the figures \ref{fig:Garnet_app_list}.

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Value_function_plot_for_safe_initial_policy_Garnet_b=50.pdf}
%          \caption{The value function at each iteration step}
%         \label{fig:gar_sp_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Cost_function_plot_for_safe_initial_policy_garnet.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:gar_sp_cf}
%     \end{subfigure}
%     \caption{The worst case value function and cost function update at each iteration step where the x-axis denotes the Iteration number and the y-axis denotes the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) denoted as Robust value function and Robust cost function respectively upon running our algorithm on the Garnet environment.}
%     \label{fig:gar_sp_cf_vf}
% \end{figure*}

% Next we test the performance of the algorithm with higher baseline such that the Markovian algorithms too can find a feasible policy. For this setting we find that for both the environments RCVI performs at par with the other algorithms.
% \subsection{Training with an elevated threshold value}
% In the following subsection, we talk about the detailed study of our algorithm along with other baselines on an elevated cost threeshold value ($b=30$ and $b=50$ for the CRS and Garnet environment respectively). Till now we observed that EPIRC-PGS and RCVI algorithms both remain in the safe-zone but the objective return of EPIRC-PGS is less. Thus, it becomes necessary to understand when we raise the threshold value, whether RCVI has comparable performance with the other baseline algorithms. The experiment plots are shown below



% From the figures \ref{fig:crs_ib_cf_vf} and \ref{fig:gar_ib_cf_vf}, we observe that EPIRC-PGS actually performs poorly in terms of objective return. In both the case RRPO aggressively increases the objective reward and for few iterations move to the unsafe zone, at this point the algorithm shifts its preference towards satisfying the constraints and steadily moves towards the safe zone. The RCRPO algorithm shows some strange behaviour for the expected cost return in the CRS environment. However,there are some policies which has similar objective rewards for example in state $s_{1},s_2,s_{3}$ the objective return is 0 despite the action taken, however, the cost is not zero, hence, there is a chance that the algorithm still learns them and due to randomness the probability transition is not fixed, however, the agent is ignorant of that and shifts its focus towards the reward as the expected cost function is below the threshold. However, such behaviour is not observed in Garnet environment since there are no similar rewarding state-action pair. This study clearly tell us, that RCVI performs in par with other markovian policy based algorithms when the threshold is high. Thus, we can infer that RCVI has the capability to find safe high returning policy for lower thresholds and perform in par with other algorithms when threshold is appropriately set making it much more reliable and efficient that other baseline algorithms.

% \subsection{Inference time (testing time) performance}
% Finally it is important to make sure the training time learning is reflected by RCVI during testing time. In this setting the results obtained during testing time are as shown in figures \ref{fig:CRS_test} and \ref{fig:Gar_test} for CRS environment and Garnet environment respectively.

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Testing_time_plot_for_RCVI_vf_CRS.pdf}
%          \caption{The value function at each iteration step}
%         \label{fig:CRS_test_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Testing_time_plot_for_RCVI_cf_CRS.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:CRS_test_cf}
%     \end{subfigure}
%     \caption{The worst case value function and cost function update at each iteration step where the x-axis denotes the Iteration number and the y-axis denotes the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) denoted as Robust value function and Robust cost function respectively upon running our algorithm on the CRS environment.}
%     \label{fig:CRS_test}
% \end{figure*}

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Testing_time_plot_for_RCVI_vf_Garnet.pdf}
%          \caption{The value function at each iteration step}
%         \label{fig:gar_test_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Testing_time_plot_for_RCVI_cf_Garnet.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:gar_test_cf}
%     \end{subfigure}
%     \caption{The worst case value function and cost function update at each iteration step where the x-axis denotes the Iteration number and the y-axis denotes the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) denoted as Robust value function and Robust cost function respectively upon running our algorithm on the Garnet environment.}
%     \label{fig:Gar_test}
% \end{figure*}

%\vspace-1em}
\section{Policy evaluation using KL-divergence as the f-divergence measure}\label{kl_divergence}
%\vspace-0.5em}
For KL divergence uncertainty set, the worst case value function can be achieved by the following expression from Proposition 5 in \cite{xu2023improved}
\begin{align}\label{eq:worst_kl}
L_{\cP_{h,x,a}}V
= -\inf_{\lambda\in[0,H/\rho]}\lambda\Big\{\rho+\log\,
\mathbb E_{x'\sim P_h^o(\cdot\mid x,a)}\!\big[e^{\big(-\frac{V(x')}{\lambda}\big)}\big]\Big\}
\end{align}
Then by Lemma 4 in \cite{iyengar2005robust} we have the worst case model for $j=r,g$ as
\begin{align}\label{eq:worst_model_kl}
P_{j,h}^*\propto P_h^0\exp(-V_{j,h+1}(x')/\lambda_j^*)
\end{align}
where $\lambda_j^*$ is the solution of the convex optimization problem in (\ref{eq:worst_kl}) for $V_{j,h}$. Note that here $x'=(s',c-g_h)$, thus, here one only needs to solve it for the state component rather than the budget evolution component. Also, (\ref{eq:worst_kl}) is a convex optimization problem. Yet, solving for all state-action pair is computationally expensive.  We thus consider an update given by \cite{Epigraph} which we adapt for the episodic case recursively starting from state $H+1$. Note that $V_{r,H+1}(\cdot,\cdot)=0$ whereas $V_{g,H+1}(\cdot,c)=-c$. 

In particular, we consider the following update
\begin{align}\label{eq:equivalent}
& Q_{g,h}(s,c,a)=\sum_{s^{\prime}}P_{g,h}^*(s^{\prime}|s,a)V_{g,h+1}(s',c-g_h),\nonumber \\&P_{g,h}^*\propto P_h^0(\cdot|s,a)\exp(-V_{g,h+1}(s',c-g_h)/C'_{g,KL}),\nonumber\\
& Q_{r,h}(s,c,a)=r_h(s,a)+\sum_{s^{\prime}}P_h^*(s^{\prime}|s,a)V_{r,h+1}(s^{\prime},c-g_h), \nonumber \\& P_{r,h}^*\propto P_h^0(\cdot|s,a)\exp(-V_{r,h+1}(s^{\prime},c-g_h)/C'_{r,KL})
\end{align}
Once we obtain $Q$ values, we will find the policy as described in Algorithm~\ref{algo:rs-cmdp}, and update the $V$-value at step $h$. 
Then by Lemma 5 in \cite{Epigraph}, for any $C'_{j,KL}>0$ there exists $\rho>0$ such that the solution in (\ref{eq:worst_kl}) converges to $\rho$ showing the equivalence. We use this expression in (\ref{eq:equivalent}) for the robust value function update. 

For RNPG, and RCRPO we use the KL-divergence evaluator adapted to the episodic case exactly as described in \cite{Epigraph} as they are policy optimization based algorithms. 
%Our algorithm assumes the existence of a robust policy evaluator oracle that evaluates $\min_{P}\mathbb{E}_{s'\sim P_h(\cdot | s, a)} \left[{V}_{g,h+1}(s',\hat{c}-(g_h(s,a)))\right]$ for a given $\pi$. There are many evaluation techniques that are used to efficiently evaluate a robust policy perturbed by popular uncertainty measures. In this work, we evaluate our policies using a variant EPIRC-PGS algorithm \cite{Epigraph} for KL uncertainty set (as shown in Algorithm \ref{algo:kl_oracle_aug}).

%The general robust DP equation is given by Equation (\ref{lab_rob_dp})

% \begin{equation}
%     \begin{aligned}
%         \textbf{(ROBUST DP): }&~Q_{c_{n}}^{(t+1)}(s,a) = c_{n}(s,a) + \min_{p \in \mathbb{P}}\sum_{s^{\prime} \in \mathcal{S}}p(s^{\prime})V_{c_{n}}^{t}(s^{\prime}),\\
%         &\text{where } V_{c_{n}}^t(s^{\prime}) := \sum_{a^{\prime}\in \mathcal{A}} \pi(s^{\prime},a^{\prime})Q_{c_{n}}^{t}(s^{\prime},a^{\prime}).
%     \end{aligned}
%     \label{lab_rob_dp}
% \end{equation}

%\textcolor{red}{KP: @ Arnob can you please take a pass at Appendix D and E to fix any notation typos? }

% \begin{algorithm}
% \caption{KL Uncertainty Evaluator}
% \label{algo:kl_oracle}
%     \begin{algorithmic}[1]
%         \STATE \textbf{Input:} policy $\pi$, nominal probability transition function $p^{0}$, perturbation parameter $\rho$, $c_{i}=\left[c_{0},c_{1},\ldots c_{K}\right]$, smoothing factor $\alpha_{kle}$,discount factor$\gamma$, $\beta$ (initial state distribution deterministic in our case), $|\mathcal{S}|,|\mathcal{A}|$
%         \STATE $Q,V$ is obtained by solving equation \ref{eqn:q_infty} iteratively.
%         \STATE $P^{*}[s,a,.]= \alpha_{kle}p^{0}[s,a,.]\exp{\left(\frac{V[.]}{\rho}\right)}~\forall(s,a) \in \mathcal{S} \times \mathcal{A}$ %\textcolor{red}{please do not use $*$ as multiplication symbol. do not even need to use $.$ if the context is clear.}
%         \STATE $T[s,s^{\prime}] = \underset{a \in \mathcal{A}}{\Sigma}\pi(a|s)P^{*}(s,a,s^{\prime}), \quad \forall (s,s^{\prime}) \in \mathcal{S} \times \mathcal{S}$
%         \STATE $Q^{\pi}_{c_{i},P^{*}} = (I-\gamma T)^{-1}c_{i}$
%         \STATE $\hat{J} = \beta^{T}\left(\underset{a \in \mathcal{A}}{\Sigma}(\pi(a|s)Q^{\pi}_{c_{i},P^{*}}(s,a))\right)$
%         % \STATE $d^{\pi}_{P^{*}} = (1-\gamma)(I-\gamma T)^{-1}\beta$
%         % \STATE $\nabla \hat{J} = Hd^{\pi}_{P^{*}}(s)Q^{\pi}_{c_{i},P^{*}}(s,a) ~~\forall ~(s,a) \in \mathcal{S} \times \mathcal{A}$
%         \STATE \textbf{Return:} $\hat{J}$
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{KL Uncertainty Evaluator for Augmented State Space}
% \label{algo:kl_oracle_aug}
% \begin{algorithmic}[1]
%     \STATE \textbf{Input:} policy $\pi(a \mid s,b)$, nominal transition model $p^{0}(s' \mid s,a)$, perturbation parameter $\rho$, cost function $c_{i}=\left[c_{0},c_{1},\ldots c_{K}\right]$, smoothing factor $\alpha_{\text{kle}}$, horizon $T$, initial state--budget distribution $\beta(s,b)$ (deterministic in our case), and sizes $|\mathcal{S}|,|\mathcal{A}|$.
%     \STATE Initialize $Q,V$ for all $(s,b) \in \mathcal{S}\times \mathcal{B}$.
%     \STATE Compute $Q,V$ by iteratively solving the robust dynamic programming equation:
%     \[
%         Q_{c_i}^{(t+1)}(s,b,a) = c_i(s,a) + \min_{p \in \mathbb{P}(s,a)} 
%         \sum_{s'\in\mathcal{S}} p(s')\, V_{c_i}^{t}(s',b - c_i(s,a)).
%     \]
%     \STATE Construct the robust transition model:
%     \[
%         P^{*}[(s,b),a,(s',b')] 
%         = \alpha_{\text{kle}}\, p^{0}(s' \mid s,a)\,
%         \exp\!\left(\frac{V(s',b')}{\rho}\right),
%     \]
%     where $b' = b - c_i(s,a)$ and infeasible $(s',b')$ pairs with $b'<0$ are ignored.
%     \STATE Compute the policy-induced transition operator:
%     \[
%         T[(s,b),(s',b')] 
%         = \sum_{a\in\mathcal{A}} \pi(a \mid s,b)\, P^{*}[(s,b),a,(s',b')].
%     \]
%     \STATE Evaluate the robust cost-to-go:
%     \[
%         Q^{\pi}_{c_i,P^{*}} = (I - T)^{-1} c_i,
%     \]
%     or for episodic horizon $T$, recursively compute backward:
%     \[
%         Q^{t}(s,b,a) = c_i(s,a) + \sum_{s'} P^{*}[(s,b),a,(s',b-c_i(s,a))]\, V^{t+1}(s',b - c_i(s,a)).
%     \]
%     \STATE Compute the performance estimate:
%     \[
%         \hat{J} = \sum_{(s,b)} \beta(s,b) 
%         \sum_{a\in\mathcal{A}} \pi(a \mid s,b)\, Q^{\pi}_{c_i,P^{*}}(s,b,a).
%     \]
%     % \STATE Compute the stationary distribution under the robust model:
%     % \[
%     %     d^{\pi}_{P^{*}} = (I - T)^{-1}\, \beta.
%     % \]
%     % \STATE Compute the policy gradient estimate:
%     % \[
%     %     \nabla \hat{J} = H\, d^{\pi}_{P^{*}}(s,b)\, Q^{\pi}_{c_i,P^{*}}(s,b,a)
%     %     \quad \forall~(s,b,a)\in \mathcal{S}\times\mathcal{B}\times\mathcal{A}.
%     % \]
%     \STATE \textbf{Return:} $\hat{J}$%, $d^{\pi}_{P^{*}}$, and $\nabla \hat{J}$.
% \end{algorithmic}
% \end{algorithm}

% \begin{equation}
% \begin{aligned}
% &\textbf{(Robust DP )}
% ~~~ Q_{c_n}^{\,t}(s,b,a)
% = c_n(s,a)
% + \begin{cases}
% \displaystyle \min_{p\in\mathbb{P}(s,a)} \sum_{s'\in\mathcal{S}} p(s')\,V_{c_n}^{\,t+1}\!\big(s',\,b-c_n(s,a)\big), 
% & b - c_n(s,a)\ge 0,\\[8pt]
% +\infty, & b - c_n(s,a) < 0,
% \end{cases}\\[8pt]
% &\qquad V_{c_n}^{\,t}(s,b)
% = \sum_{a\in\mathcal{A}} \pi_t(a\mid s,b)\; Q_{c_n}^{\,t}(s,b,a), \qquad t=0,\dots,T-1,\\[6pt]
% %&\qquad V_{c_n}^{\,T}(s,b)= -\,b \qquad\text{(terminal value; alternative terminal convention possible).}
% \end{aligned}
% \label{lab_rob_dp}
% \end{equation}

% \begin{equation*}
%     \begin{aligned}
%         \mathbb{P} = \otimes_{s,a} \mathbb{P}_{(s,a)} \quad\text{where} \quad \mathbb{P}_{(s,a)} = \{P \in \Delta(\mathcal{S}) | \mathrm{KL}\left[P|P_0(.|s,a)\right]\leq \rho\},
%     \end{aligned}
% \end{equation*}
% where $\mathbb{P}$ satisfies $(s,a)$-rectangularity assumption and $\mathrm{KL}[p|q] = \sum_{s\in \mathcal{S}} p(s) \ln{\frac{p(s)}{q(s)}}$ for two probability distribution $p,q \in \Delta(\mathcal{S})$. The KL uncertainty evaluator (see Algorithm \ref{algo:kl_oracle_aug}) is justified by Lemma 4 and 5 in \cite{Epigraph}.


% \textcolor{red}{KP: @ Sourav, adding as a comment instead of me fixing all instances. Please capitalize Algorithm or Lemma references when using them.}
%The KL uncertainty evaluator follows from a variant of Lemma~\ref{lem:kl_uncertainty_evalutor} as explained in section \ref{app:extension}.  %In Algorithm \ref{algo:kl_oracle}, we need the Robust\_Q-table. The compact algorithm for that is given in Algorithm \ref{algo:rq_tab}.
% \begin{algorithm}[h]
% \caption{Robust\_Q-table}
% \label{algo:rq_tab}
%     \begin{algorithmic}[1]
%     \STATE \textbf{Input:} $c_{i},\pi,p^0,\rho,\rho$, smoothing factor $\alpha$
%     \STATE \textbf{Initialize:} $Q(s,a)=0 ~\forall (s,a) \in \mathcal{S}\times \mathcal{A}$, $V(s)=0~\forall s \in \mathcal{S}, Q_{prev}(s,a)=0~~\forall (s,a) \in \mathcal{S}\times \mathcal{A}$
%     % \STATE $\tau \to \infty$
%     \STATE $s = \rho(.),~\tau = 1000,~i=1$
%     \WHILE{$i < \tau$ }
%     \STATE $Q_{prev}(s,a) = Q(s,a)~~\forall (s,a) \in \mathcal{S}\times \mathcal{A}$
%     \STATE $a = \pi(.|s)$
%     \STATE $s^{\prime}=p^{0}(.|s,a)$
%     \STATE $P^{*} = p^{0}(s,a,.)\exp{\left(\alpha\frac{V[.]}{\rho}\right)}$
%     \STATE $Q[s,a] = c_{i}[s,a]+\gamma\langle P^{*},V\rangle$
%     \STATE $V[s] = \langle\pi[.|s],Q(s,.)\rangle ~~\forall s \in \mathcal{S}$
%     \STATE $s=s^{\prime}$
%     \IF{$Q(s,a)=Q_{prev}(s,a) ~~\forall (s,a) \in \mathcal{S}\times \mathcal{A}$}
%     \STATE Break out of loop
%     \ENDIF
%     \STATE $i=i+1$
%     \ENDWHILE
%     \STATE \textbf{Return:} $Q,~V$
%     \end{algorithmic}
% \end{algorithm}
% \begin{lemma}\label{lem:kl_uncertainty_evalutor}
%     (\textbf{Lemma 4} in \cite{iyengar2005robust}) Let $v \in \mathbb{R}^{|\mathcal{S}|}$ and $0 <q <\Delta(\mathcal{S})$. The value of optimization problem
%     \begin{equation}
%         \underset{p \in  \Delta(\mathcal{S})}{\min} \langle p,v\rangle~ such~ that~KL[p||q]<C_{KL} 
%         \label{eqn:supl1}
%     \end{equation}
%     is equal to
%     \begin{align}
%         \min_{\theta\geq 0} \theta C_{KL} +\theta\ln{(\langle q,\exp{(-\frac{v}{\theta})}\rangle)}.
%         \label{eqn:supl2}
%     \end{align}
%     Let $\theta^{*}$ be the solution of equation (\ref{eqn:supl2}), then the solution of \eqref{eqn:supl1} becomes,
%     \begin{equation}
%         p \propto q\exp{(-\frac{v}{\theta^{*}})}.
%     \end{equation}
%     \label{lem:supl1}
% \end{lemma}

% Using lemma \ref{lem:supl1}, Equation \eqref{lab_rob_dp} can be implemented as
% \begin{equation}
%     \begin{aligned}
%         &Q_{c_{n}}^{(t+1)}(s,a) = c_{n}(s,a)+\gamma\sum_{s \in \mathcal{S}}P^{*}_{(s,a)}(s^{\prime})V_{c_{n}}^{(t)}(s^{\prime}),\\
%         &\text{where } P^{*}_{(s,a)} \propto p^{0}(.|s,a)\exp{\left(\frac{V_{c_{n}}^{t}(.)}{\theta^{*}_{(s,a)}}\right)},\\
%         &\text{and }\theta^{*}_{(s,a)}:=\arg\min_{\theta\geq 0} \theta C_{KL}+\theta\ln{\left(\langle p^{0}(.|s,a),\exp\left(\frac{V_{c_{n}}^{t}(.)}{\theta} \right) \rangle\right)}.
%     \end{aligned}
%     \label{eqn:supl3}
% \end{equation}

% While Equation \eqref{eqn:supl2} is convex in nature, solving it for all $p(.|s,a) \forall(s,a) \in (\mathcal{S},\mathcal{A})$ in Equation \eqref{eqn:supl3} is computationally extensive in practice. Rather than the exact constrained problem, \cite{yang2023robustmarkovdecisionprocesses} proposed a \textbf{regularized robust DP update}. 

% \begin{equation}
%     \begin{aligned}
%         Q_{c_{n}}^{(t+1)}(s,a) = c_{n}(s,a) + \gamma \underset{p \in \Delta_{\mathcal{S}}}{\max}\left( \sum_{s^{\prime}\in \mathcal{S}}p(s^{\prime})V_{c_{n}}^{t}(s^{\prime}) - C_{KL}^{'}KL[p||p^{0}(.|s,a)]\right),
%     \end{aligned}
%     \label{eqn:supl4}
% \end{equation}
% where $C^{'}_{KL}>0$ is a constant. This regularized form can be efficiently written as Equation \eqref{eqn:q_infty}
% \begin{equation}
%     \begin{aligned}
%         Q_{c_{n}}^{(t+1)} = c_{n}(s,a) + \gamma \left(\underset{s^{\prime} \in \mathcal{S}}{\Sigma} P^{*}_{(s,a)} (s^{\prime})V_{c_{n}}^{t}(s^{\prime}) \right),\\
%         \text{where  } P^{*}_{(s,a)} \propto p^{0}(.|s,a)\exp{\left(\frac{V_{c_{n}}^{t}(.)}{C^{'}_{KL}} \right)}.
%     \end{aligned}
%     \label{eqn:q_infty}
% \end{equation}
% The equivalence can be concluded from the duality since it is convex optimization problem. The following lemma also shows that the convergence is fast.
% \begin{lemma}
%     (Adaptation from \textbf{Proposition 3.1} and \textbf{Theorem 3.1} \cite{yang2023robustmarkovdecisionprocesses}) For any $C_{KL}^{'}>0$, there exists $\rho>0$ such that Equation \eqref{eqn:supl4} converges linearly to the fixed point of Equation \eqref{eqn:supl3}.
%     \label{lem:supl2}
% \end{lemma}
% \subsection{KL-Robust Dynamic Programming for Augmented State Space}
% \label{app:extension}

% We extend Lemma~4 from \cite{iyengar2005robust} to the augmented state space 
% $\tilde{\mathcal{S}} = \mathcal{S} \times \mathcal{B}$, where each augmented state 
% $\tilde{s} = (s, b)$ represents the environment state $s \in \mathcal{S}$ and the 
% remaining budget $b \in \mathcal{B}$.

% \begin{lemma}[KL-Uncertainty Evaluator for Augmented State Space]
% \label{lem:aug_kl}
% Let $v \in \mathbb{R}^{|\tilde{\mathcal{S}}|}$ and 
% $q \in \Delta(\tilde{\mathcal{S}})$ denote a nominal probability distribution 
% over augmented next states. Consider the following constrained optimization problem:
% \begin{equation}
%     \min_{p \in \Delta(\tilde{\mathcal{S}})} 
%     \langle p, v \rangle 
%     \quad \text{s.t.} \quad 
%     \mathrm{KL}(p \,\|\, q) \leq C_{KL}.
%     \label{eq:aug_min_problem}
% \end{equation}
% Then, the optimal value of~\eqref{eq:aug_min_problem} is given by the one-dimensional convex optimization:
% \begin{equation}
%     \min_{\theta \geq 0} 
%     \; \theta C_{KL} 
%     + \theta \ln 
%     \Big( \langle q, \exp(-v / \theta) \rangle \Big),
%     \label{eq:aug_dual_form}
% \end{equation}
% and the corresponding optimal solution $p^{*}$ takes the exponential-tilting form:
% \begin{equation}
%     p^{*}(\tilde{s}') 
%     = \frac{ q(\tilde{s}') \, \exp(-v(\tilde{s}') / \theta^{*}) }
%            { \sum_{\tilde{s}'' \in \tilde{\mathcal{S}}} 
%            q(\tilde{s}'') \, \exp(-v(\tilde{s}'') / \theta^{*}) },
%     \label{eq:aug_p_star}
% \end{equation}
% where $\theta^{*}$ is the optimal solution to~\eqref{eq:aug_dual_form}.
% \end{lemma}

% \begin{proof}
% The proof follows directly from the Lagrangian dual formulation of 
% KL-constrained minimization as in \cite{iyengar2005robust}. 
% The key difference here is that $p, q \in \Delta(\tilde{\mathcal{S}})$ 
% are distributions over the augmented state space. 
% Replacing $\mathcal{S}$ by $\tilde{\mathcal{S}}$ in Lemma~4 of 
% \cite{iyengar2005robust} yields the same dual representation 
% in~\eqref{eq:aug_dual_form} and the corresponding exponential form 
% in~\eqref{eq:aug_p_star}.
% \end{proof}

% \paragraph{Application to Robust Dynamic Programming.}
% We now apply Lemma~\ref{lem:aug_kl} to the robust Bellman update 
% in the augmented state space.  
% Let $\tilde{s} = (s, b)$ denote the current augmented state and $a \in \mathcal{A}$ 
% an action. The corresponding one-step cost is $c_{n}(s, a)$ and the nominal 
% transition distribution on augmented states is defined as
% \begin{equation}
%     q(\tilde{s}' = (s', b') \mid s, b, a) 
%     =
%     \begin{cases}
%         p^{0}(s' \mid s, a), & \text{if } b' = b - c_{n}(s, a) \ge 0, \\[3pt]
%         0, & \text{otherwise.}
%     \end{cases}
%     \label{eq:aug_nominal_trans}
% \end{equation}

% The robust Bellman update for the augmented state space is then:
% \begin{equation}
%     Q_{c_{n}}^{(t+1)}(s, b, a)
%     = c_{n}(s, a)
%     + \min_{p \in \Delta(\tilde{\mathcal{S}})} 
%       \sum_{\tilde{s}' \in \tilde{\mathcal{S}}} 
%       p(\tilde{s}') \, V_{c_{n}}^{(t)}(\tilde{s}'),
%     \label{eq:aug_robust_dp}
% \end{equation}
% where $V_{c_{n}}^{(t)}(\tilde{s}') 
% = \sum_{a'} \pi(a' \mid \tilde{s}') Q_{c_{n}}^{(t)}(\tilde{s}', a')$.

% Applying Lemma~\ref{lem:aug_kl} to the inner minimization in~\eqref{eq:aug_robust_dp}, 
% we obtain the optimal adversarial distribution:
% \begin{equation}
%     p^{*}_{(s,b,a)}(\tilde{s}')
%     = 
%     \frac{
%         q(\tilde{s}' \mid s,b,a)
%         \exp\!\left(-V_{c_{n}}^{(t)}(\tilde{s}') / \theta^{*}_{(s,b,a)}\right)
%     }{
%         \sum_{\tilde{s}''}
%         q(\tilde{s}'' \mid s,b,a)
%         \exp\!\left(-V_{c_{n}}^{(t)}(\tilde{s}'') / \theta^{*}_{(s,b,a)}\right)
%     },
%     \label{eq:aug_p_star_final}
% \end{equation}
% where $\theta^{*}_{(s,b,a)}$ solves:
% \begin{equation}
%     \theta^{*}_{(s,b,a)} 
%     = \arg\min_{\theta \ge 0}
%       \left[
%         \theta C_{KL}
%         + \theta \ln
%         \Big\langle 
%             q(\cdot \mid s,b,a), 
%             \exp\!\left(-V_{c_{n}}^{(t)}(\cdot)/\theta\right)
%         \Big\rangle
%       \right].
%     \label{eq:aug_theta_star}
% \end{equation}

% Substituting~\eqref{eq:aug_p_star_final} into~\eqref{eq:aug_robust_dp}, we get the 
% final KL-robust Bellman recursion for the augmented state space:
% \begin{equation}
%     Q_{c_{n}}^{(t+1)}(s, b, a)
%     = c_{n}(s, a)
%     + \sum_{\tilde{s}' \in \tilde{\mathcal{S}}} 
%       p^{*}_{(s,b,a)}(\tilde{s}') \,
%       V_{c_{n}}^{(t)}(\tilde{s}'),
%     \label{eq:aug_final_robust_dp}
% \end{equation}
% and
% \begin{equation}
%     V_{c_{n}}^{(t)}(s, b) 
%     = \sum_{a \in \mathcal{A}} 
%       \pi(a \mid s, b) \, Q_{c_{n}}^{(t)}(s, b, a).
%     \label{eq:aug_value_func}
% \end{equation}

% \paragraph{Remarks.}
% \begin{itemize}
%     \item The term $\exp(-V/\theta)$ ensures the minimization of expected value under KL-divergence uncertainty, 
%     aligning with the worst-case adversarial dynamics.
%     \item The parameter $\theta^{*}_{(s,b,a)}$ balances robustness and nominal optimality — 
%     smaller $\theta^{*}$ yields higher conservativeness.
%     \item The nominal kernel $q(\tilde{s}' \mid s,b,a)$ in~\eqref{eq:aug_nominal_trans} 
%     automatically enforces budget feasibility by assigning zero probability mass to 
%     infeasible successors $(s',b')$ where $b' < 0$.
% \end{itemize}
% =====================================================================
%  PROOF APPENDIX (IEEE layout: each part is a \subsection, so it is
%  referenced as "Appendix C", "Appendix D", ...).
%
%  Place this right after the experiment appendices (CRS and Garnet).
%  It REPLACES everything in the current draft from "C. Proof of Lemma
%  III.1" to the end, and ALSO the old TV proof of Lemma 2.1 that now sits
%  at the end of the Garnet ablation subsection (Fig. 9 and the "Proof."
%  paragraph after it). Keep Fig. 9 if you like, and move it into the
%  Lemma 2.1 part below.
%
%  Do NOT keep any of the following from the current draft; each is
%  either a duplicate or incorrect:
%   - Section D's Fact 2, the re-definition of F, Assumption A.2,
%     Lemmas A.3-A.5, Theorem A.6, Remark A.1 (old numbers), Remark A.7
%     (duplicates of Section IV and of the proof part below);
%   - Section E "Proof of Theorem 3.1" (Theorem A.8, Remark A.9): it claims
%     Markov policies on (s,c) are sufficient for the RCMDP, which is not
%     proved and is false as stated (pi-star need not keep the state in F).
% =====================================================================

==> partial_details_necessary.tex <==
\subsection{Additional experiments and experiment details}
\label{app:experiments}
We use KL-divergence as the $f$-divergence metric due to its closed-form evaluation for a known nominal model $P_0$ and its stability across hyperparameter changes. Although the method extends to other $f$-divergences, such as TV and $\chi^2$-divergence, we focus on KL-divergence. Uncertainty is introduced by perturbing and normalizing the nominal transition probabilities during training, with the perturbation reversed during testing on Constrained Riverswim(CRS) and Cost based Garnet environments (Refer to \cite{ganguly2025provablyefficientsamplecomplexity} for more experiments and discussion).
% The experiments were performed on two very popular benchmarks in RL\footnote{Lower threshold experiments ($b=4.5$ for RCVI in CRS) were done in colab without use of hardware accelerators such as GPU or TPU for higher threshold $b=30$ for CRS and for Garnet are done in a local machine, having 4GB RAM and 1 TB of hard disk, no GPU support is necessary.} (i) Constrained River-swim (CRS) and (ii) Cost-based Garnet environment. For both the experiments, the f-divergence metric is assumed to be KL-divergence. Although the algorithm is not limited to KL-divergence and can be extended to other f-divergence measures such as TV-distance, $\chi^{2}$-distribution etc.  There are two important reasons for choosing the KL-divergence over the other f-divergence metrics. First the existence of a closed form evaluation method that makes the robust policy evaluation having a known nominal model ($P_{0}$), simple (see Appendix \ref{kl_divergence}). Secondly, the KL-divergence is very stable with minimum influence of the changing hyperparameters. The uncertainty is introduced in both environments by adding noise to the nominal model transition probabilities and then normalizing them to make a probability distribution during training time and by reversing the probability distribution in the testing or inference time.

% \subsubsection{Constrained River-swim}
% % The constrained River-swim (CRS) is an important benchmark environment studied in optimization theory and control. We briefly introduce the objective of the Constrained River-swim environment, followed by the results obtained upon training our algorithm (Algorithm \ref{algo:rs-cmdp}) on CRS.

% % \subsubsection{Environment Description}
% We consider a six-state RiverSwim environment\cite{ganguly2025provablyefficientsamplecomplexity}. Rewards are concentrated at the extreme states, while safety costs increase with the state index due to river currents and harmful creatures. The agent therefore learns a reward-maximizing policy subject to a safety budget under transition uncertainty.



% \subsubsection{Additional Results and discussion}
% % The results obtained upon training Algorithm \ref{algo:rs-cmdp} on CRS is as shown in figures \ref{fig:CRS_vf_app} and \ref{fig:CRS_cf_app}
% In addition to the experiments reported in Figure~\ref{fig:crs_ib_cf_vf_main}, we conduct several supplementary experiments to further illustrate the limitations of the Markovian policy setup and the advantages of the augmented formulation.

% The choice of budget threshold $b=4.5$ may appear unconventional and could raise questions regarding its selection. Our motivation, however, is deliberate: we choose $b$ so that none of the competing algorithms can identify a feasible policy under this budget. This helps expose a fundamental limitation of the Markovian setup, namely its inability to recover feasible policies when all candidate policies lie in the unsafe region, a limitation that does not arise in the augmented setting.

%As an alternative way to demonstrate this phenomenon, we also increase the cost at every state by $0.5$. Figures~\ref{fig:CRS_vf_app}, \ref{fig:CRS_cf_app}, \ref{fig:CRS_app_inc_cost_vf}, and \ref{fig:CRS_app_inc_cost_cf} show the results for this modified cost function relative to the costs reported in Table~\ref{tab:rs_r_c}. \textcolor{red}{Note that we omit RRPO and EPIRC-PGS from these plots because their values were too close to distinguish clearly.}

%The reason RCVI does not violate the threshold in either setup stems from its discretization of cost budget over the range $[0,b]$. Since RCVI only permits decisions within this discretized budget space, the agent cannot select actions that lead beyond the prescribed cost bound. In contrast, the other algorithms do not impose any analogous budget discretization or bucket structure and instead update parameters iteratively without an explicit mechanism guaranteeing feasibility. Consequently, when all candidate policies lie in the unsafe region, these methods have no way to recover a feasible policy. %To explicitly demonstrate this limitation, we choose the challenging threshold $b=4.5$ in Figures~\ref{fig:crs_ib_cf_vf_main} and \ref{fig:CRS_app_list}.

% \begin{figure}
%     \centering
%     \begin{subfigure}
%         \includegraphics[]{images/Aistats_VI_vf.pdf}
%         \caption{The value function at each iteration step}
%         \label{fig:CRS_vf}
%     \end{subfigure}

%     \begin{subfigure}
%         \includegraphics[]{images/Aistats_VI_cf.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:CRS_cf}
%     \end{subfigure}
%     \caption{The worst case value function and cost function update at each iteration step where the x-axis denotes the Iteration number and the y-axis denots the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) denoted as Robust value function and Robust cost function respectively.}
%     \label{fig:CRS}
% \end{figure}

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[clip=2in 2in 2in 2in,height=2.3in]{images/Comparison_plots_rho_1e-1_baseline_reducedCRSvf.pdf}
%          \caption{The value function at each iteration step}
%         \label{fig:CRS_vf_app}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[clip=2in 2in 2in 2in,height=2.3in]{images/Comparison_plots_rho_1e-1_baseline_reducedCRSCF.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:CRS_cf_app}
%     \end{subfigure}
%     \caption{The Robust value function and Robust cost function update (CRS environment) at each iteration step , the baseline kept as 5 and cost at each step is increased by $0.5$ with respect to table \ref{tab:rs_r_c} ($\rho=0.01$)}
%     \label{fig:CRS_app_1}
% \end{figure*}

% The baseline for the cost function ($b$) or the budget was fixed at $4.5$.  As seen in figure \ref{fig:CRS_vf_app}, the value function steadily increases to the maximum possible in the given budget range. Starting from $0.24$ approximately which denotes the robust value function for the policy of equiprobable actions in each states (i.e $\pi(a|s) = \frac{1}{|\mathcal{A}|}~\forall s\in \mathcal{S}$), it slowly increases and after 50 iterations it converges to the policy where the robust value function is maximum. As it is evident that the convergence is faster compared to other state-of-the approaches. Further, the RCVI (Algorithm~\ref{algo:rs-cmdp}) is always feasible.   The implementation details along with the hyperparameters are listed in the following subsection. %(Since, the baseline staright line and the RCVI cost function plot is nearly coinciding refer to figure \ref{zoom_in_CRS_cf} for better demonstration).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{images/Comparison_plots_rho_1e-1_inc_cost_zoom_CRSCF.pdf}
%     \caption{Robust cost function update at each iteration on CRS environment (baseline =4.5 and zoomed in to show how many times RCVI cost function goes past the baseline)}
%     \label{zoom_in_CRS_cf}
% \end{figure}

%In another set of experiments on CRS environment, we increased the baseline by $0.5$, that is the new baseline was set at $5$ (we also ran one set of experiment by fixing the baseline at 7 and keeping all other hyper-parameters, rewards and cost intact as this experiment and results were almost similar). However, we increased the cost at each state denoted by Table \ref{tab:rs_r_c} by $0.5$. This experiment was performed as a control experiment to verify if RNPG or RCRPO perform in par with RCVI. The results of which are depicted in figures \ref{fig:CRS_app_inc_cost_vf} and \ref{fig:CRS_app_inc_cost_cf}.

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[clip=2in 2in 2in 2in,height=2.3in]{images/Comparison_plots_rho_1e-2_increased_costCRSvf.pdf}
%          \caption{The value function at each iteration step}
%         \label{fig:CRS_app_inc_cost_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[clip=2in 2in 2in 2in,height=2.3in]{images/Comparison_plots_rho_1e-2_increased_costCRSCF.pdf}
%         \caption{The cost function at each iteration step}
%         \label{fig:CRS_app_inc_cost_cf}
%     \end{subfigure}
%     \caption{\small The Robust value function and Robust cost function update (CRS environment) at each iteration step , the baseline kept as 5 and cost at each step is increased by $0.5$ with respect to table \ref{tab:rs_r_c} ($\rho=0.1$)}
%     \label{fig:CRS_app_2}
% \end{figure*}

% \paragraph{Test Time  results} 
% \label{testing_CRS}
% Since our training procedure incorporates robustness, it is important to verify whether these benefits persist at inference (test) time under perturbed dynamics. To evaluate this, we deliberately perturb the transition probabilities during testing. Specifically, if the agent is at state $s_t=x$, it can transition to one of $s_{t+1}=\{x-1,x,x+1\}$ with probabilities $p_1,p_2,p_3$, respectively. During testing, with probability $\epsilon$, we randomly alter the transition ordering; for example, the transition probabilities may change from $(p_1,p_2,p_3)$ to $(p_3,p_2,p_1)$. For our test-time, we set $\epsilon=0.05$.

%  We initialize from random states, sample actions from the learned Q-table using the same cost discretization, and run a reduced evaluation over $100$ independent episodes. We then report the average robust value function and robust cost function, summarized in Table~\ref{tab:robust_results}.
% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|}
%     \hline
%         \textbf{Environment name}&\textbf{RCVI} &RNPG&RRPO&EPIRC-PGS&RCRPO  \\
%         \hline
%         \textit{CRS}&\textbf{5.5044} &6.0456&5.00031& 14.113&12.7812\\
%         \hline
%          \textit{Garnet}&\textbf{4.4081}&8.2304&6.00214&9.211&11.5488 \\
%          \hline
%     \end{tabular}
%     \caption{Average robust value functions of 100 steps for all the algorithms on the two environments}
%     \label{tab:testing_vf}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%         \textbf{RCVI} &RNPG&RRPO&EPIRC-PGS&RCRPO   \\
%         \hline
%          \textit{CRS}&\textbf{4.4081}&8.2304&6.00214&9.211&11.5488 \\
%          \hline
         
%     \end{tabular}
%     \caption{Average robust cost functions of 100 steps for all the algorithms,  $b=4.5$.}
%     \label{tab:testing_cf_CRS}
% \end{table}
% \subsubsection{Training with an increased safety threshold value}
% \paragraph{Training with a safety threshold $b=7$} In addition to the above setup, we run our algorithm with a higher safety threshold value to underscore the performance of RCVI. We first consider $b=7$ and $\rho=0.1$.  Since $b$ is high, now the Markovian policies in the original state-space is feasible, yet we observe that our proposed approach (RCVI) converges faster compared to the other baselines (Figure~\ref{fig:one_safe_pol_crs}).   From Figure \ref{one_safe_pol_crs_vf}, we note that all the algorithms have comparable value functions, and Figure \ref{one_safe_pol_crs_cf} tells us that all the algorithms are in the safe zone. %Hence, we can conclude that RCVI  returns a high-returning (comparable to other baselines) feasible policy.

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.2in]{images/Baseline_where_one_policy_in_safe_zone_vf_CRS.pdf}
%          \caption{The value function at each iteration step}
%         \label{one_safe_pol_crs_vf}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.2in]{Baseline_where_one_policy_in_safe_zone_cf_CRS.pdf}
%         \caption{The cost function at each iteration step}
%         \label{one_safe_pol_crs_cf}
%     \end{subfigure}
%     \caption{\small Robust value function and cost function update at each iteration on Constrained River-swim(CRS environment) $b=7$.}
%     %\vspace-0.2in}
%     \label{fig:one_safe_pol_crs}
% \end{figure*}

% \paragraph{Training with a safety threshold $b=30$}
% In addition to the above setup, we run our algorithm with a higher safety threshold value to underscore the performance of RCVI. We consider threshold $b=30$ and $\rho=0.1$. Here, the Markovian policy in the original state-space is feasible, and all the other baselines converge to the optimal policy as well. In this setup too, we find that the convergence of RCVI is faster compared to other state-of-the-art approaches (Figure~\ref{fig:crs_ib_cf_vf}. RCVI also achieves a similar reward while maintaining feasibility throughout the training. {\em This set of studies  tell us that RCVI can  not only find a feasible policy but also the highest-returning feasible policy across different values of $b$}. Further, RCVI converges  faster compared to  all the state-of-the-art approaches.  
\begin{figure*}[h!]
    \centering
    \begin{subfigure}[h]{0.4\textwidth}
        \centering
        \includegraphics[height=1.7in]{images/Value_function_plot_for_safe_initial_policy_CRS_b=30.pdf}
         \caption{\small The value function at each iteration step}
        \label{fig:crs_ib_vf}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[h]{0.4\textwidth}
        \centering
        \includegraphics[height=1.7in]{images/Cost_function_plot_for_safe_initial_policy_CRS_b=30.pdf}
        \caption{\small The cost function at each iteration step}
        \label{fig:crs_ib_cf}
    \end{subfigure}
    \caption{\small Robust value function and cost function update at each iteration on Constrained River-swim (CRS) environment for $b=30$.}
    \label{fig:crs_ib_cf_vf}
\end{figure*}
%\vspace-0.1in}
\paragraph{Ablation study on uncertainty measure $\rho$ for CRS environment}
In this section, we perform an ablation study on different values of $\rho$ for the CRS environment (original setting). The results of which can be found in Figure \ref{fig:CRS_app_list} where we compare with the baselines.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.65\textwidth]{images/Ablation_CRS_rho_0.01_0.1.pdf}
    \caption{\small Worst-case reward vs Iteration (left) and worst case cost vs Iteration (right) for different values of $\rho$.}
    \label{fig:CRS_app_list}
\end{figure*}

% \begin{figure*}[]
%     \centering
%     \begin{subfigure}[]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.01_vf.pdf}
%          \caption{The value function at each iteration step ($\rho=0.01$)}
%         \label{fig:CRS_vf_app_0.01}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.01_cf.pdf}
%         \caption{The cost function at each iteration step ($\rho=0.01$)}
%         \label{fig:CRS_cf_app_0.01}
%     \end{subfigure}%
%      \\
%     % \begin{subfigure}[]{0.5\textwidth}
%     %     \centering
%     %     \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.05_vf.pdf}
%     %     \caption{The value function at each iteration step($\rho=0.05$)}
%     %     \label{fig:CRS_vf_app_0.05}
%     % \end{subfigure}%
%     % ~
%     % \begin{subfigure}[]{0.5\textwidth}
%     %     \centering
%     %     \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.05_cf.pdf}
%     %     \caption{The cost function at each iteration step($\rho=0.05$)}
%     %     \label{fig:CRS_cf_app_0.05}
%     % \end{subfigure}%
%     % \\
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.1_vf.pdf}
%          \caption{The value function at each iteration step($\rho=0.1$)}
%         \label{fig:CRS_vf_app_0.1}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[h]{0.5\textwidth}
%         \centering
%         \includegraphics[height=2.3in]{images/Ablation_CRS_rho_0.1_cf.pdf}
%         \caption{The cost function at each iteration step($\rho=0.1$)}
%         \label{fig:CRS_cf_app_0.1}
%     \end{subfigure}
%     %  \begin{subfigure}[]{0.5\textwidth}
%     %     \centering
%     %     \includegraphics[height=2.3in]{images/Abalation_CRS_rho_0.05_vf.pdf}
%     %      \caption{The value function at each iteration step ($\rho=0.05$)}
%     %     \label{fig:CRS_vf_app_0.1}
%     % \end{subfigure}%
%     % ~ 
%     % \begin{subfigure}[]{0.5\textwidth}
%     %     \centering
%     %     \includegraphics[height=2.3in]{images/Ablataion_CRS_rho_0.05_cf.pdf}
%     %     \caption{The cost function at each iteration step ($\rho=0.05$)}
%     %     \label{fig:CRS_cf_app_0.1}
%     % \end{subfigure}%
%    % \begin{subfigure}[h]{0.5\textwidth}
%    %      \centering
%    %      \includegraphics[height=2.8in]{images/Aistats_VI_vf_Garnet.pdf}
%    %       \caption{The value function at each iteration step }
%    %      \label{app:fig_gar_vf}
%    %  \end{subfigure}%
%    %  ~ 
%    %  \begin{subfigure}[h]{0.5\textwidth}
%    %      \centering
%    %      \includegraphics[height=2.8in]{images/Aistats_VI_cf_Garnet.pdf}
%    %      \caption{The cost function at each iteration step($\rho=0.5$)}
%    %      \label{app:fig_gar_cf}
%    %  \end{subfigure}
%     \caption{\small Worst-case reward vs Iteration (left) and worst case cost vs Iteration (right) for different values of $\rho$.}
%     \label{fig:CRS_app_list}
% \end{figure*}

The first row of plots (Figures~\ref{fig:CRS_app_list}) corresponds to $\rho = 0.01$ and the final row of plots correspond to $\rho=0.1$. The baseline was kept at $4.5$ for all the experiments. In all cases, baseline algorithms such as RNPG, RRPO, RCRPO, and EPIRC-PGS operate in the unsafe region, requiring large iterations to converge. In contrast, our RCVI algorithm consistently remains within the safe boundary,  and converges to the optimal policy quickly.% Moreover, for $\rho=0.1$ (Figure~\ref{fig:CRS_vf_app_0.1}) the achieved value function is slightly higher compared to RNPG.

\subsubsection{Cost-based Garnet problem}
 For our experiments, we set \(B=15\), use \(20\) bins, \(H=N=1000\), and \(f\)-divergence tolerance \(\rho\in\{0.01,0.05,0.1\}\).


% \subsubsection{Additional Results and discussion}
% Similar to the CRS environment, we conduct additional experiments to support the advantages of our approach. The choice of budget for most of the pilot studies, the testing time study, and the ablation study was 15.
% % \begin{figure*}[h!]
% %     \centering
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.2in]{Comparison_plots_rho_1e-1_icmlGarnetvf.pdf}
% %          \caption{The value function at each iteration step}
% %         \label{app:fig_gar_vf}
% %     \end{subfigure}%
% %     ~ 
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.2in]{Comparison_plots_rho_1e-1_icmlGarnetCF.pdf}
% %         \caption{The cost function at each iteration step}
% %         \label{app:fig_gar_cf}
% %     \end{subfigure}
% %     \caption{The worst case value function and cost function (garnet environment) update at each iteration step where the x-axis denotes the Iteration number and the y-axis denotes the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) with the cost at each state randomly increased by $Unif(0,0.5)$.}
% %     \label{fig:garnet_app}
% % \end{figure*}

% \paragraph{Testing Time (Inference time) results}
% \label{testing_garnet}
% During test time, we run $100$ independent episodes where the initial state is chosen randomly. The average robust value function and average robust cost function are listed in tables \ref{tab:robust_results}. Only the RCVI achieves a feasible policy while also achieving a good reward. 



% % \begin{table}[h!]
% %     \centering
% %     \begin{tabular}{|c|c|c|c|c|}
% %     \hline
% %         \textbf{RCVI} &RNPG&RRPO&EPIRC-PGS&RCRPO  \\
% %         \hline
% %         \textbf{21.0125} &22.9541&20.1546& 20.5441&31.1546\\
% %         \hline
% %     \end{tabular}
% %     \caption{\small Average robust value functions of 100 steps for all the algorithms (Garnet environment)}
% %     \label{tab:rvf_garnet}
% % \end{table}

% % \begin{table}[h!]
% %     \centering
% %     \begin{tabular}{|c|c|c|c|c|}
% %     \hline
% %         \textbf{RCVI} &RNPG&RRPO&EPIRC-PGS&RCRPO   \\
% %         \hline
% %          \textbf{14.9562}&23.5541&19.8456&22.7741&24.1179 \\
% %          \hline
         
% %     \end{tabular}
% %     \caption{\small Average robust cost functions of 100 steps for all the algorithms (Garnet environment), $b=15$.}
% %     \label{tab:rcf_garnet}
% % \end{table}
% \subsubsection{Training with an increased safety threshold value}
% % \paragraph{Training with a safety threshold $b=25$}  We begin by studying a slightly higher baseline $b=25$. The findings from this study are compiled in Figures \ref{one_safe_pol_garnet_vf} and \ref{one_safe_pol_garnet_cf}. 
% % \begin{figure*}[h!]
% %     \centering
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.2in]{images/Baseline_where_one_policy_in_safe_zone_vf_garnet.pdf}
% %          \caption{The value function at each iteration step}
% %         \label{one_safe_pol_garnet_vf}
% %     \end{subfigure}%
% %     ~ 
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.2in]{images/Baseline_where_one_policy_in_safe_zone_cf_garnet.pdf}
% %         \caption{The cost function at each iteration step}
% %         \label{one_safe_pol_garnet_cf}
% %     \end{subfigure}
% %     \caption{The above plot shows when only 1 policy exists in the feasible zone then all other algorithms finds that policy however, our RCVI algorithm is still effective in such situations (Garnet environment) $b=25$.}
% %     \label{fig:one_safe_pol_garnet}
% % \end{figure*}
% % Since $b$ is high, the Markovian policies are also feasible. As observed from Figure \ref{fig:one_safe_pol_garnet}, all the algorithms converge to a close enough policy with  comparable value function and cost functions. However, our proposed approach RCVI coverges the fastest among all the other approaches. 

% Similar to CRS, for this envionment too, we try with an elevated baseline value $b=50$. From Figure~\ref{fig:gar_ib_cf_vf} note that our proposed approach is the fastest among all the other approaches. The achieved reward is almost similar with the baselines while maintaining feasibility throughout the training. %The plots for this study is shown in figure \ref{fig:gar_ib_cf_vf}.

\begin{figure*}[h!]
    \centering
    \begin{subfigure}[h]{0.4\textwidth}
        \centering
        \includegraphics[clip=2in 2in 2in 2in,height=1.7in]{images/Value_function_plot_for_safe_initial_policy_Garnet_b=50.pdf}
         \caption{The value function at each iteration step}
        \label{fig:gar_ib_vf}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[h]{0.4\textwidth}
        \centering
        \includegraphics[height=1.7in]{images/Cost_function_plot_for_safe_initial_policy_Garnet_b=50.pdf}
        \caption{The cost function at each iteration step}
        \label{fig:gar_ib_cf}
    \end{subfigure}
    \caption{\small Robust value function and cost function update at each iteration on Garnet environment (b=50).}
    \label{fig:gar_ib_cf_vf}
\end{figure*}

%As seen from figure \ref{fig:gar_ib_cf_vf}, RCVI performs in par with other algorithms. Thus, we can draw the inference from this experiment that RCVI performs efficiently in large baseline conditions as well.

% Evaluating both environments, despite their similar uncertainty estimators and indices, strengthens the robustness and generalizability of the results across different settings.

% \paragraph{Ablation study on uncertainty measure $\rho$}
% %\vspace-0.1in}
% Similar to the CRS setting, we conduct an ablation study on different values of $\rho$ for the Garnet environment. 
% %The uncertainty parameter $\rho$ plays a crucial role in shaping the policy search space, as varying $\rho$ alters the set of admissible policies. To understand the impact of this hyperparameter, we systematically evaluate performance across different values of $\rho$. 
% The corresponding results are presented in Figure \ref{fig:Garnet_app_list}. In all cases, baseline algorithms such as RNPG, RRPO, RCRPO, and EPIRC-PGS operate in the unsafe region, requiring large iterations to converge. In contrast, our RCVI algorithm consistently remains within the safe boundary,  and converges to the optimal policy quickly.
% %The cost budget was kept at 5, since higher values might require higher discretizations to perform best.  


% % \begin{figure*}[]
% %     \centering
% %     \begin{subfigure}[]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.01_vf.pdf}
% %          \caption{The value function at each iteration step ($\rho=0.01$)}
% %         \label{app:fig_gar_vf_0.01}
% %     \end{subfigure}%
% %     ~ 
% %     \begin{subfigure}[]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.01_cf.pdf}
% %         \caption{The cost function at each iteration step ($\rho=0.01$)}
% %         \label{app:fig_gar_cf_0.01}
% %     \end{subfigure}
% %     % \\
% %     % \begin{subfigure}[]{0.5\textwidth}
% %     %     \centering
% %     %     \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.05_vf.pdf}
% %     %      \caption{The value function at each iteration step ($\rho=0.05$)}
% %     %     \label{app:fig_gar_vf_0.05}
% %     % \end{subfigure}%
% %     % ~ 
% %     % \begin{subfigure}[]{0.5\textwidth}
% %     %     \centering
% %     %     \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.05_cf.pdf}
% %     %     \caption{The cost function at each iteration step ($\rho=0.05$)}
% %     %     \label{app:fig_gar_cf_0.05}
% %     % \end{subfigure}
% %     \\
% %      \begin{subfigure}[]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.1_vf.pdf}
% %          \caption{The value function at each iteration step ($\rho=0.1$)}
% %         \label{app:fig_gar_vf_0.1}
% %     \end{subfigure}%
% %     ~ 
% %     \begin{subfigure}[]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Ablation_Garnet_rho_0.1_cf.pdf}
% %         \caption{The cost function at each iteration step ($\rho=0.1$)}
% %         \label{app:fig_gar_cf_0.1}
% %     \end{subfigure}
% %     % \begin{subfigure}[]{0.5\textwidth}
% %     %     \centering
% %     %     \includegraphics[height=2.3in]{images/Comparison_plots_rho_1e-1_Garnetvf.pdf}
% %     %      \caption{The value function at each iteration step ($\rho=0.1$)}
% %     %     \label{app:fig_gar_vf_0.1}
% %     % \end{subfigure}%
% %     % ~ 
% %     % \begin{subfigure}[]{0.5\textwidth}
% %     %     \centering
% %     %     \includegraphics[height=2.3in]{images/Comparison_plots_rho_1e-1_GarnetCF.pdf}
% %     %     \caption{The cost function at each iteration step ($\rho=0.1$)}
% %     %     \label{app:fig_gar_cf_0.1}
% %     % \end{subfigure}
% %     \caption{\small Worst-case reward vs Iterations(left) and Worst-case cost vs Iteration (right) for different values of $\rho$.}
% %     \label{fig:Garnet_app_list}
% % \end{figure*}
% % \subsection{More Experimental results}
% %We further understand the working of our algorithm and here are the results obtained below
% % \begin{figure*}[h!]
% %     \centering
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Value_function_plot_for_safe_initial_policy_CRS.pdf}
% %          \caption{The value function at each iteration step}
% %         \label{fig:crs_sp_vf}
% %     \end{subfigure}%
% %     ~ 
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Cost_function_plot_for_safe_initial_policy_CRS.pdf}
% %         \caption{The cost function at each iteration step}
% %         \label{fig:crs_sp_cf}
% %     \end{subfigure}
% %     \caption{The worst case value function and cost function update upon running our algorithm and other baselines on the CRS environment.}
% %     \label{fig:crs_sp_cf_vf}
% % \end{figure*}

% % Figures \ref{fig:Garnet_app_list} shows a detailed comparison when all the algorithms start from the safe zone, we see only RCVI converges to a safe feasible high returning policy due to its structure while others although start safe, after the parameters gets fixed, they converge to a non-feasible policy. This is because, the baseline was deliberately kept such that none of the policies could satisfy. Even for a higher value of $\rho$, RCVI can achieve a feasible policy while the other algorithms cannot.  %With very small learning rate too the agents quickly move out of safe zone. % A similar pattern is observed in the Garnet environment which is evident from the figures \ref{fig:Garnet_app_list}.

% % \begin{figure*}[h!]
% %     \centering
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Value_function_plot_for_safe_initial_policy_Garnet_b=50.pdf}
% %          \caption{The value function at each iteration step}
% %         \label{fig:gar_sp_vf}
% %     \end{subfigure}%
% %     ~ 
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Cost_function_plot_for_safe_initial_policy_garnet.pdf}
% %         \caption{The cost function at each iteration step}
% %         \label{fig:gar_sp_cf}
% %     \end{subfigure}
% %     \caption{The worst case value function and cost function update at each iteration step where the x-axis denotes the Iteration number and the y-axis denotes the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) denoted as Robust value function and Robust cost function respectively upon running our algorithm on the Garnet environment.}
% %     \label{fig:gar_sp_cf_vf}
% % \end{figure*}

% % Next we test the performance of the algorithm with higher baseline such that the Markovian algorithms too can find a feasible policy. For this setting we find that for both the environments RCVI performs at par with the other algorithms.
% % \subsection{Training with an elevated threshold value}
% % In the following subsection, we talk about the detailed study of our algorithm along with other baselines on an elevated cost threeshold value ($b=30$ and $b=50$ for the CRS and Garnet environment respectively). Till now we observed that EPIRC-PGS and RCVI algorithms both remain in the safe-zone but the objective return of EPIRC-PGS is less. Thus, it becomes necessary to understand when we raise the threshold value, whether RCVI has comparable performance with the other baseline algorithms. The experiment plots are shown below



% % From the figures \ref{fig:crs_ib_cf_vf} and \ref{fig:gar_ib_cf_vf}, we observe that EPIRC-PGS actually performs poorly in terms of objective return. In both the case RRPO aggressively increases the objective reward and for few iterations move to the unsafe zone, at this point the algorithm shifts its preference towards satisfying the constraints and steadily moves towards the safe zone. The RCRPO algorithm shows some strange behaviour for the expected cost return in the CRS environment. However,there are some policies which has similar objective rewards for example in state $s_{1},s_2,s_{3}$ the objective return is 0 despite the action taken, however, the cost is not zero, hence, there is a chance that the algorithm still learns them and due to randomness the probability transition is not fixed, however, the agent is ignorant of that and shifts its focus towards the reward as the expected cost function is below the threshold. However, such behaviour is not observed in Garnet environment since there are no similar rewarding state-action pair. This study clearly tell us, that RCVI performs in par with other markovian policy based algorithms when the threshold is high. Thus, we can infer that RCVI has the capability to find safe high returning policy for lower thresholds and perform in par with other algorithms when threshold is appropriately set making it much more reliable and efficient that other baseline algorithms.

% % \subsection{Inference time (testing time) performance}
% % Finally it is important to make sure the training time learning is reflected by RCVI during testing time. In this setting the results obtained during testing time are as shown in figures \ref{fig:CRS_test} and \ref{fig:Gar_test} for CRS environment and Garnet environment respectively.

% % \begin{figure*}[h!]
% %     \centering
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Testing_time_plot_for_RCVI_vf_CRS.pdf}
% %          \caption{The value function at each iteration step}
% %         \label{fig:CRS_test_vf}
% %     \end{subfigure}%
% %     ~ 
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Testing_time_plot_for_RCVI_cf_CRS.pdf}
% %         \caption{The cost function at each iteration step}
% %         \label{fig:CRS_test_cf}
% %     \end{subfigure}
% %     \caption{The worst case value function and cost function update at each iteration step where the x-axis denotes the Iteration number and the y-axis denotes the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) denoted as Robust value function and Robust cost function respectively upon running our algorithm on the CRS environment.}
% %     \label{fig:CRS_test}
% % \end{figure*}

% % \begin{figure*}[h!]
% %     \centering
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Testing_time_plot_for_RCVI_vf_Garnet.pdf}
% %          \caption{The value function at each iteration step}
% %         \label{fig:gar_test_vf}
% %     \end{subfigure}%
% %     ~ 
% %     \begin{subfigure}[h]{0.5\textwidth}
% %         \centering
% %         \includegraphics[height=2.3in]{images/Testing_time_plot_for_RCVI_cf_Garnet.pdf}
% %         \caption{The cost function at each iteration step}
% %         \label{fig:gar_test_cf}
% %     \end{subfigure}
% %     \caption{The worst case value function and cost function update at each iteration step where the x-axis denotes the Iteration number and the y-axis denotes the worst case value function at that iteration (left figure) and the worst case cost function at that iteration (right figure) denoted as Robust value function and Robust cost function respectively upon running our algorithm on the Garnet environment.}
% %     \label{fig:Gar_test}
% % \end{figure*}

% %\vspace-1em}
% \subsection{Policy evaluation using KL-divergence as the f-divergence measure}\label{kl_divergence}
% %\vspace-0.5em}
% For KL divergence uncertainty set, the worst case value function can be achieved by the following expression from Proposition 5 in \cite{xu2023improved}
% \begin{align}\label{eq:worst_kl}
% L_{\cP_{h,x,a}}V
% = -\inf_{\lambda\in[0,H/\rho]}\lambda\Big\{\rho+\log\,
% \mathbb E_{x'\sim P_h^o(\cdot\mid x,a)}\!\big[e^{\big(-\frac{V(x')}{\lambda}\big)}\big]\Big\}
% \end{align}
% Then by Lemma 4 in \cite{iyengar2005robust} we have the worst case model for $j=r,g$ as
% \begin{align}\label{eq:worst_model_kl}
% P_{j,h}^*\propto P_h^0\exp(-V_{j,h+1}(x')/\lambda_j^*)
% \end{align}
% where $\lambda_j^*$ is the solution of the convex optimization problem in (\ref{eq:worst_kl}) for $V_{j,h}$. Note that here $x'=(s',c-g_h)$, thus, here one only needs to solve it for the state component rather than the budget evolution component. Also, (\ref{eq:worst_kl}) is a convex optimization problem. Yet, solving for all state-action pair is computationally expensive.  We thus consider an update given by \cite{Epigraph} which we adapt for the episodic case recursively starting from state $H+1$. Note that $V_{r,H+1}(\cdot,\cdot)=0$ whereas $V_{g,H+1}(\cdot,c)=-c$. 

% In particular, we consider the following update
% \begin{align}\label{eq:equivalent}
% & Q_{g,h}(s,c,a)=\sum_{s^{\prime}}P_{g,h}^*(s^{\prime}|s,a)V_{g,h+1}(s',c-g_h),\nonumber \\&P_{g,h}^*\propto P_h^0(\cdot|s,a)\exp(-V_{g,h+1}(s',c-g_h)/C'_{g,KL}),\nonumber\\
% & Q_{r,h}(s,c,a)=r_h(s,a)+\sum_{s^{\prime}}P_h^*(s^{\prime}|s,a)V_{r,h+1}(s^{\prime},c-g_h), \nonumber \\& P_{r,h}^*\propto P_h^0(\cdot|s,a)\exp(-V_{r,h+1}(s^{\prime},c-g_h)/C'_{r,KL})
% \end{align}
% Once we obtain $Q$ values, we will find the policy as described in Algorithm~\ref{algo:rs-cmdp}, and update the $V$-value at step $h$. 
% Then by Lemma 5 in \cite{Epigraph}, for any $C'_{j,KL}>0$ there exists $\rho>0$ such that the solution in (\ref{eq:worst_kl}) converges to $\rho$ showing the equivalence. We use this expression in (\ref{eq:equivalent}) for the robust value function update. 

% For RNPG, and RCRPO we use the KL-divergence evaluator adapted to the episodic case exactly as described in \cite{Epigraph} as they are policy optimization based algorithms. 
% %Our algorithm assumes the existence of a robust policy evaluator oracle that evaluates $\min_{P}\mathbb{E}_{s'\sim P_h(\cdot | s, a)} \left[{V}_{g,h+1}(s',\hat{c}-(g_h(s,a)))\right]$ for a given $\pi$. There are many evaluation techniques that are used to efficiently evaluate a robust policy perturbed by popular uncertainty measures. In this work, we evaluate our policies using a variant EPIRC-PGS algorithm \cite{Epigraph} for KL uncertainty set (as shown in Algorithm \ref{algo:kl_oracle_aug}).

% %The general robust DP equation is given by Equation (\ref{lab_rob_dp})

% % \begin{equation}
% %     \begin{aligned}
% %         \textbf{(ROBUST DP): }&~Q_{c_{n}}^{(t+1)}(s,a) = c_{n}(s,a) + \min_{p \in \mathbb{P}}\sum_{s^{\prime} \in \mathcal{S}}p(s^{\prime})V_{c_{n}}^{t}(s^{\prime}),\\
% %         &\text{where } V_{c_{n}}^t(s^{\prime}) := \sum_{a^{\prime}\in \mathcal{A}} \pi(s^{\prime},a^{\prime})Q_{c_{n}}^{t}(s^{\prime},a^{\prime}).
% %     \end{aligned}
% %     \label{lab_rob_dp}
% % \end{equation}

% %\textcolor{red}{KP: @ Arnob can you please take a pass at Appendix D and E to fix any notation typos? }

% % \begin{algorithm}
% % \caption{KL Uncertainty Evaluator}
% % \label{algo:kl_oracle}
% %     \begin{algorithmic}[1]
% %         \STATE \textbf{Input:} policy $\pi$, nominal probability transition function $p^{0}$, perturbation parameter $\rho$, $c_{i}=\left[c_{0},c_{1},\ldots c_{K}\right]$, smoothing factor $\alpha_{kle}$,discount factor$\gamma$, $\beta$ (initial state distribution deterministic in our case), $|\mathcal{S}|,|\mathcal{A}|$
% %         \STATE $Q,V$ is obtained by solving equation \ref{eqn:q_infty} iteratively.
% %         \STATE $P^{*}[s,a,.]= \alpha_{kle}p^{0}[s,a,.]\exp{\left(\frac{V[.]}{\rho}\right)}~\forall(s,a) \in \mathcal{S} \times \mathcal{A}$ %\textcolor{red}{please do not use $*$ as multiplication symbol. do not even need to use $.$ if the context is clear.}
% %         \STATE $T[s,s^{\prime}] = \underset{a \in \mathcal{A}}{\Sigma}\pi(a|s)P^{*}(s,a,s^{\prime}), \quad \forall (s,s^{\prime}) \in \mathcal{S} \times \mathcal{S}$
% %         \STATE $Q^{\pi}_{c_{i},P^{*}} = (I-\gamma T)^{-1}c_{i}$
% %         \STATE $\hat{J} = \beta^{T}\left(\underset{a \in \mathcal{A}}{\Sigma}(\pi(a|s)Q^{\pi}_{c_{i},P^{*}}(s,a))\right)$
% %         % \STATE $d^{\pi}_{P^{*}} = (1-\gamma)(I-\gamma T)^{-1}\beta$
% %         % \STATE $\nabla \hat{J} = Hd^{\pi}_{P^{*}}(s)Q^{\pi}_{c_{i},P^{*}}(s,a) ~~\forall ~(s,a) \in \mathcal{S} \times \mathcal{A}$
% %         \STATE \textbf{Return:} $\hat{J}$
% %     \end{algorithmic}
% % \end{algorithm}

% % \begin{algorithm}[H]
% % \caption{KL Uncertainty Evaluator for Augmented State Space}
% % \label{algo:kl_oracle_aug}
% % \begin{algorithmic}[1]
% %     \STATE \textbf{Input:} policy $\pi(a \mid s,b)$, nominal transition model $p^{0}(s' \mid s,a)$, perturbation parameter $\rho$, cost function $c_{i}=\left[c_{0},c_{1},\ldots c_{K}\right]$, smoothing factor $\alpha_{\text{kle}}$, horizon $T$, initial state--budget distribution $\beta(s,b)$ (deterministic in our case), and sizes $|\mathcal{S}|,|\mathcal{A}|$.
% %     \STATE Initialize $Q,V$ for all $(s,b) \in \mathcal{S}\times \mathcal{B}$.
% %     \STATE Compute $Q,V$ by iteratively solving the robust dynamic programming equation:
% %     \[
% %         Q_{c_i}^{(t+1)}(s,b,a) = c_i(s,a) + \min_{p \in \mathbb{P}(s,a)} 
% %         \sum_{s'\in\mathcal{S}} p(s')\, V_{c_i}^{t}(s',b - c_i(s,a)).
% %     \]
% %     \STATE Construct the robust transition model:
% %     \[
% %         P^{*}[(s,b),a,(s',b')] 
% %         = \alpha_{\text{kle}}\, p^{0}(s' \mid s,a)\,
% %         \exp\!\left(\frac{V(s',b')}{\rho}\right),
% %     \]
% %     where $b' = b - c_i(s,a)$ and infeasible $(s',b')$ pairs with $b'<0$ are ignored.
% %     \STATE Compute the policy-induced transition operator:
% %     \[
% %         T[(s,b),(s',b')] 
% %         = \sum_{a\in\mathcal{A}} \pi(a \mid s,b)\, P^{*}[(s,b),a,(s',b')].
% %     \]
% %     \STATE Evaluate the robust cost-to-go:
% %     \[
% %         Q^{\pi}_{c_i,P^{*}} = (I - T)^{-1} c_i,
% %     \]
% %     or for episodic horizon $T$, recursively compute backward:
% %     \[
% %         Q^{t}(s,b,a) = c_i(s,a) + \sum_{s'} P^{*}[(s,b),a,(s',b-c_i(s,a))]\, V^{t+1}(s',b - c_i(s,a)).
% %     \]
% %     \STATE Compute the performance estimate:
% %     \[
% %         \hat{J} = \sum_{(s,b)} \beta(s,b) 
% %         \sum_{a\in\mathcal{A}} \pi(a \mid s,b)\, Q^{\pi}_{c_i,P^{*}}(s,b,a).
% %     \]
% %     % \STATE Compute the stationary distribution under the robust model:
% %     % \[
% %     %     d^{\pi}_{P^{*}} = (I - T)^{-1}\, \beta.
% %     % \]
% %     % \STATE Compute the policy gradient estimate:
% %     % \[
% %     %     \nabla \hat{J} = H\, d^{\pi}_{P^{*}}(s,b)\, Q^{\pi}_{c_i,P^{*}}(s,b,a)
% %     %     \quad \forall~(s,b,a)\in \mathcal{S}\times\mathcal{B}\times\mathcal{A}.
% %     % \]
% %     \STATE \textbf{Return:} $\hat{J}$%, $d^{\pi}_{P^{*}}$, and $\nabla \hat{J}$.
% % \end{algorithmic}
% % \end{algorithm}

% % \begin{equation}
% % \begin{aligned}
% % &\textbf{(Robust DP )}
% % ~~~ Q_{c_n}^{\,t}(s,b,a)
% % = c_n(s,a)
% % + \begin{cases}
% % \displaystyle \min_{p\in\mathbb{P}(s,a)} \sum_{s'\in\mathcal{S}} p(s')\,V_{c_n}^{\,t+1}\!\big(s',\,b-c_n(s,a)\big), 
% % & b - c_n(s,a)\ge 0,\\[8pt]
% % +\infty, & b - c_n(s,a) < 0,
% % \end{cases}\\[8pt]
% % &\qquad V_{c_n}^{\,t}(s,b)
% % = \sum_{a\in\mathcal{A}} \pi_t(a\mid s,b)\; Q_{c_n}^{\,t}(s,b,a), \qquad t=0,\dots,T-1,\\[6pt]
% % %&\qquad V_{c_n}^{\,T}(s,b)= -\,b \qquad\text{(terminal value; alternative terminal convention possible).}
% % \end{aligned}
% % \label{lab_rob_dp}
% % \end{equation}

% % \begin{equation*}
% %     \begin{aligned}
% %         \mathbb{P} = \otimes_{s,a} \mathbb{P}_{(s,a)} \quad\text{where} \quad \mathbb{P}_{(s,a)} = \{P \in \Delta(\mathcal{S}) | \mathrm{KL}\left[P|P_0(.|s,a)\right]\leq \rho\},
% %     \end{aligned}
% % \end{equation*}
% % where $\mathbb{P}$ satisfies $(s,a)$-rectangularity assumption and $\mathrm{KL}[p|q] = \sum_{s\in \mathcal{S}} p(s) \ln{\frac{p(s)}{q(s)}}$ for two probability distribution $p,q \in \Delta(\mathcal{S})$. The KL uncertainty evaluator (see Algorithm \ref{algo:kl_oracle_aug}) is justified by Lemma 4 and 5 in \cite{Epigraph}.


% % \textcolor{red}{KP: @ Sourav, adding as a comment instead of me fixing all instances. Please capitalize Algorithm or Lemma references when using them.}
% %The KL uncertainty evaluator follows from a variant of Lemma~\ref{lem:kl_uncertainty_evalutor} as explained in section \ref{app:extension}.  %In Algorithm \ref{algo:kl_oracle}, we need the Robust\_Q-table. The compact algorithm for that is given in Algorithm \ref{algo:rq_tab}.
% % \begin{algorithm}[h]
% % \caption{Robust\_Q-table}
% % \label{algo:rq_tab}
% %     \begin{algorithmic}[1]
% %     \STATE \textbf{Input:} $c_{i},\pi,p^0,\rho,\rho$, smoothing factor $\alpha$
% %     \STATE \textbf{Initialize:} $Q(s,a)=0 ~\forall (s,a) \in \mathcal{S}\times \mathcal{A}$, $V(s)=0~\forall s \in \mathcal{S}, Q_{prev}(s,a)=0~~\forall (s,a) \in \mathcal{S}\times \mathcal{A}$
% %     % \STATE $\tau \to \infty$
% %     \STATE $s = \rho(.),~\tau = 1000,~i=1$
% %     \WHILE{$i < \tau$ }
% %     \STATE $Q_{prev}(s,a) = Q(s,a)~~\forall (s,a) \in \mathcal{S}\times \mathcal{A}$
% %     \STATE $a = \pi(.|s)$
% %     \STATE $s^{\prime}=p^{0}(.|s,a)$
% %     \STATE $P^{*} = p^{0}(s,a,.)\exp{\left(\alpha\frac{V[.]}{\rho}\right)}$
% %     \STATE $Q[s,a] = c_{i}[s,a]+\gamma\langle P^{*},V\rangle$
% %     \STATE $V[s] = \langle\pi[.|s],Q(s,.)\rangle ~~\forall s \in \mathcal{S}$
% %     \STATE $s=s^{\prime}$
% %     \IF{$Q(s,a)=Q_{prev}(s,a) ~~\forall (s,a) \in \mathcal{S}\times \mathcal{A}$}
% %     \STATE Break out of loop
% %     \ENDIF
% %     \STATE $i=i+1$
% %     \ENDWHILE
% %     \STATE \textbf{Return:} $Q,~V$
% %     \end{algorithmic}
% % \end{algorithm}
% % \begin{lemma}\label{lem:kl_uncertainty_evalutor}
% %     (\textbf{Lemma 4} in \cite{iyengar2005robust}) Let $v \in \mathbb{R}^{|\mathcal{S}|}$ and $0 <q <\Delta(\mathcal{S})$. The value of optimization problem
% %     \begin{equation}
% %         \underset{p \in  \Delta(\mathcal{S})}{\min} \langle p,v\rangle~ such~ that~KL[p||q]<C_{KL} 
% %         \label{eqn:supl1}
% %     \end{equation}
% %     is equal to
% %     \begin{align}
% %         \min_{\theta\geq 0} \theta C_{KL} +\theta\ln{(\langle q,\exp{(-\frac{v}{\theta})}\rangle)}.
% %         \label{eqn:supl2}
% %     \end{align}
% %     Let $\theta^{*}$ be the solution of equation (\ref{eqn:supl2}), then the solution of \eqref{eqn:supl1} becomes,
% %     \begin{equation}
% %         p \propto q\exp{(-\frac{v}{\theta^{*}})}.
% %     \end{equation}
% %     \label{lem:supl1}
% % \end{lemma}

% % Using lemma \ref{lem:supl1}, Equation \eqref{lab_rob_dp} can be implemented as
% % \begin{equation}
% %     \begin{aligned}
% %         &Q_{c_{n}}^{(t+1)}(s,a) = c_{n}(s,a)+\gamma\sum_{s \in \mathcal{S}}P^{*}_{(s,a)}(s^{\prime})V_{c_{n}}^{(t)}(s^{\prime}),\\
% %         &\text{where } P^{*}_{(s,a)} \propto p^{0}(.|s,a)\exp{\left(\frac{V_{c_{n}}^{t}(.)}{\theta^{*}_{(s,a)}}\right)},\\
% %         &\text{and }\theta^{*}_{(s,a)}:=\arg\min_{\theta\geq 0} \theta C_{KL}+\theta\ln{\left(\langle p^{0}(.|s,a),\exp\left(\frac{V_{c_{n}}^{t}(.)}{\theta} \right) \rangle\right)}.
% %     \end{aligned}
% %     \label{eqn:supl3}
% % \end{equation}

% % While Equation \eqref{eqn:supl2} is convex in nature, solving it for all $p(.|s,a) \forall(s,a) \in (\mathcal{S},\mathcal{A})$ in Equation \eqref{eqn:supl3} is computationally extensive in practice. Rather than the exact constrained problem, \cite{yang2023robustmarkovdecisionprocesses} proposed a \textbf{regularized robust DP update}. 

% % \begin{equation}
% %     \begin{aligned}
% %         Q_{c_{n}}^{(t+1)}(s,a) = c_{n}(s,a) + \gamma \underset{p \in \Delta_{\mathcal{S}}}{\max}\left( \sum_{s^{\prime}\in \mathcal{S}}p(s^{\prime})V_{c_{n}}^{t}(s^{\prime}) - C_{KL}^{'}KL[p||p^{0}(.|s,a)]\right),
% %     \end{aligned}
% %     \label{eqn:supl4}
% % \end{equation}
% % where $C^{'}_{KL}>0$ is a constant. This regularized form can be efficiently written as Equation \eqref{eqn:q_infty}
% % \begin{equation}
% %     \begin{aligned}
% %         Q_{c_{n}}^{(t+1)} = c_{n}(s,a) + \gamma \left(\underset{s^{\prime} \in \mathcal{S}}{\Sigma} P^{*}_{(s,a)} (s^{\prime})V_{c_{n}}^{t}(s^{\prime}) \right),\\
% %         \text{where  } P^{*}_{(s,a)} \propto p^{0}(.|s,a)\exp{\left(\frac{V_{c_{n}}^{t}(.)}{C^{'}_{KL}} \right)}.
% %     \end{aligned}
% %     \label{eqn:q_infty}
% % \end{equation}
% % The equivalence can be concluded from the duality since it is convex optimization problem. The following lemma also shows that the convergence is fast.
% % \begin{lemma}
% %     (Adaptation from \textbf{Proposition 3.1} and \textbf{Theorem 3.1} \cite{yang2023robustmarkovdecisionprocesses}) For any $C_{KL}^{'}>0$, there exists $\rho>0$ such that Equation \eqref{eqn:supl4} converges linearly to the fixed point of Equation \eqref{eqn:supl3}.
% %     \label{lem:supl2}
% % \end{lemma}
% % \subsection{KL-Robust Dynamic Programming for Augmented State Space}
% % \label{app:extension}

% % We extend Lemma~4 from \cite{iyengar2005robust} to the augmented state space 
% % $\tilde{\mathcal{S}} = \mathcal{S} \times \mathcal{B}$, where each augmented state 
% % $\tilde{s} = (s, b)$ represents the environment state $s \in \mathcal{S}$ and the 
% % remaining budget $b \in \mathcal{B}$.

% % \begin{lemma}[KL-Uncertainty Evaluator for Augmented State Space]
% % \label{lem:aug_kl}
% % Let $v \in \mathbb{R}^{|\tilde{\mathcal{S}}|}$ and 
% % $q \in \Delta(\tilde{\mathcal{S}})$ denote a nominal probability distribution 
% % over augmented next states. Consider the following constrained optimization problem:
% % \begin{equation}
% %     \min_{p \in \Delta(\tilde{\mathcal{S}})} 
% %     \langle p, v \rangle 
% %     \quad \text{s.t.} \quad 
% %     \mathrm{KL}(p \,\|\, q) \leq C_{KL}.
% %     \label{eq:aug_min_problem}
% % \end{equation}
% % Then, the optimal value of~\eqref{eq:aug_min_problem} is given by the one-dimensional convex optimization:
% % \begin{equation}
% %     \min_{\theta \geq 0} 
% %     \; \theta C_{KL} 
% %     + \theta \ln 
% %     \Big( \langle q, \exp(-v / \theta) \rangle \Big),
% %     \label{eq:aug_dual_form}
% % \end{equation}
% % and the corresponding optimal solution $p^{*}$ takes the exponential-tilting form:
% % \begin{equation}
% %     p^{*}(\tilde{s}') 
% %     = \frac{ q(\tilde{s}') \, \exp(-v(\tilde{s}') / \theta^{*}) }
% %            { \sum_{\tilde{s}'' \in \tilde{\mathcal{S}}} 
% %            q(\tilde{s}'') \, \exp(-v(\tilde{s}'') / \theta^{*}) },
% %     \label{eq:aug_p_star}
% % \end{equation}
% % where $\theta^{*}$ is the optimal solution to~\eqref{eq:aug_dual_form}.
% % \end{lemma}

% % \begin{proof}
% % The proof follows directly from the Lagrangian dual formulation of 
% % KL-constrained minimization as in \cite{iyengar2005robust}. 
% % The key difference here is that $p, q \in \Delta(\tilde{\mathcal{S}})$ 
% % are distributions over the augmented state space. 
% % Replacing $\mathcal{S}$ by $\tilde{\mathcal{S}}$ in Lemma~4 of 
% % \cite{iyengar2005robust} yields the same dual representation 
% % in~\eqref{eq:aug_dual_form} and the corresponding exponential form 
% % in~\eqref{eq:aug_p_star}.
% % \end{proof}

% % \paragraph{Application to Robust Dynamic Programming.}
% % We now apply Lemma~\ref{lem:aug_kl} to the robust Bellman update 
% % in the augmented state space.  
% % Let $\tilde{s} = (s, b)$ denote the current augmented state and $a \in \mathcal{A}$ 
% % an action. The corresponding one-step cost is $c_{n}(s, a)$ and the nominal 
% % transition distribution on augmented states is defined as
% % \begin{equation}
% %     q(\tilde{s}' = (s', b') \mid s, b, a) 
% %     =
% %     \begin{cases}
% %         p^{0}(s' \mid s, a), & \text{if } b' = b - c_{n}(s, a) \ge 0, \\[3pt]
% %         0, & \text{otherwise.}
% %     \end{cases}
% %     \label{eq:aug_nominal_trans}
% % \end{equation}

% % The robust Bellman update for the augmented state space is then:
% % \begin{equation}
% %     Q_{c_{n}}^{(t+1)}(s, b, a)
% %     = c_{n}(s, a)
% %     + \min_{p \in \Delta(\tilde{\mathcal{S}})} 
% %       \sum_{\tilde{s}' \in \tilde{\mathcal{S}}} 
% %       p(\tilde{s}') \, V_{c_{n}}^{(t)}(\tilde{s}'),
% %     \label{eq:aug_robust_dp}
% % \end{equation}
% % where $V_{c_{n}}^{(t)}(\tilde{s}') 
% % = \sum_{a'} \pi(a' \mid \tilde{s}') Q_{c_{n}}^{(t)}(\tilde{s}', a')$.

% % Applying Lemma~\ref{lem:aug_kl} to the inner minimization in~\eqref{eq:aug_robust_dp}, 
% % we obtain the optimal adversarial distribution:
% % \begin{equation}
% %     p^{*}_{(s,b,a)}(\tilde{s}')
% %     = 
% %     \frac{
% %         q(\tilde{s}' \mid s,b,a)
% %         \exp\!\left(-V_{c_{n}}^{(t)}(\tilde{s}') / \theta^{*}_{(s,b,a)}\right)
% %     }{
% %         \sum_{\tilde{s}''}
% %         q(\tilde{s}'' \mid s,b,a)
% %         \exp\!\left(-V_{c_{n}}^{(t)}(\tilde{s}'') / \theta^{*}_{(s,b,a)}\right)
% %     },
% %     \label{eq:aug_p_star_final}
% % \end{equation}
% % where $\theta^{*}_{(s,b,a)}$ solves:
% % \begin{equation}
% %     \theta^{*}_{(s,b,a)} 
% %     = \arg\min_{\theta \ge 0}
% %       \left[
% %         \theta C_{KL}
% %         + \theta \ln
% %         \Big\langle 
% %             q(\cdot \mid s,b,a), 
% %             \exp\!\left(-V_{c_{n}}^{(t)}(\cdot)/\theta\right)
% %         \Big\rangle
% %       \right].
% %     \label{eq:aug_theta_star}
% % \end{equation}

% % Substituting~\eqref{eq:aug_p_star_final} into~\eqref{eq:aug_robust_dp}, we get the 
% % final KL-robust Bellman recursion for the augmented state space:
% % \begin{equation}
% %     Q_{c_{n}}^{(t+1)}(s, b, a)
% %     = c_{n}(s, a)
% %     + \sum_{\tilde{s}' \in \tilde{\mathcal{S}}} 
% %       p^{*}_{(s,b,a)}(\tilde{s}') \,
% %       V_{c_{n}}^{(t)}(\tilde{s}'),
% %     \label{eq:aug_final_robust_dp}
% % \end{equation}
% % and
% % \begin{equation}
% %     V_{c_{n}}^{(t)}(s, b) 
% %     = \sum_{a \in \mathcal{A}} 
% %       \pi(a \mid s, b) \, Q_{c_{n}}^{(t)}(s, b, a).
% %     \label{eq:aug_value_func}
% % \end{equation}

% % \paragraph{Remarks.}
% % \begin{itemize}
% %     \item The term $\exp(-V/\theta)$ ensures the minimization of expected value under KL-divergence uncertainty, 
% %     aligning with the worst-case adversarial dynamics.
% %     \item The parameter $\theta^{*}_{(s,b,a)}$ balances robustness and nominal optimality — 
% %     smaller $\theta^{*}$ yields higher conservativeness.
% %     \item The nominal kernel $q(\tilde{s}' \mid s,b,a)$ in~\eqref{eq:aug_nominal_trans} 
% %     automatically enforces budget feasibility by assigning zero probability mass to 
% %     infeasible successors $(s',b')$ where $b' < 0$.
% % \end{itemize}
% % =====================================================================
% %  PROOF APPENDIX (IEEE layout: each part is a \subsection, so it is
% %  referenced as "Appendix C", "Appendix D", ...).
% %
% %  Place this right after the experiment appendices (CRS and Garnet).
% %  It REPLACES everything in the current draft from "C. Proof of Lemma
% %  III.1" to the end, and ALSO the old TV proof of Lemma 2.1 that now sits
% %  at the end of the Garnet ablation subsection (Fig. 9 and the "Proof."
% %  paragraph after it). Keep Fig. 9 if you like, and move it into the
% %  Lemma 2.1 part below.
% %
% %  Do NOT keep any of the following from the current draft; each is
% %  either a duplicate or incorrect:
% %   - Section D's Fact 2, the re-definition of F, Assumption A.2,
% %     Lemmas A.3-A.5, Theorem A.6, Remark A.1 (old numbers), Remark A.7
% %     (duplicates of Section IV and of the proof part below);
% %   - Section E "Proof of Theorem 3.1" (Theorem A.8, Remark A.9): it claims
% %     Markov policies on (s,c) are sufficient for the RCMDP, which is not
% %     proved and is false as stated (pi-star need not keep the state in F).
% % =====================================================================

==> tmlr/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

